Active Token Mixer

The three existing dominant network families, i.e., CNNs, Transformers, and MLPs, differ from each other mainly in the ways of fusing spatial contextual information, leaving designing more effective token-mixing mechanisms at the core of backbone architecture development. In this work, we propose an innovative token-mixer, dubbed Active Token Mixer (ATM), to actively incorporate flexible contextual information distributed across different channels from other tokens into the given query token. This fundamental operator actively predicts where to capture useful contexts and learns how to fuse the captured contexts with the query token at channel level. In this way, the spatial range of token-mixing can be expanded to a global scope with limited computational complexity, where the way of token-mixing is reformed. We take ATM as the primary operator and assemble ATMs into a cascade architecture, dubbed ATMNet. Extensive experiments demonstrate that ATMNet is generally applicable and comprehensively surpasses different families of SOTA vision backbones by a clear margin on a broad range of vision tasks, including visual recognition and dense prediction tasks. Code is available at https://github.com/microsoft/ActiveMLP.

==> tables/ade20k.tex <==
\begingroup
\small
\resizebox{0.475\textwidth}{!}{
\begin{NiceTabular}{@{}lcccc@{}}[code-before=
\rectanglecolor{\rc}{2-1}{2-15}
\rectanglecolor{\rc}{8-1}{8-15}
\rectanglecolor{\rc}{14-1}{14-15}
\rectanglecolor{\rc}{20-1}{21-15}
]
\toprule
% Backbone & \makecell{\#P.\\(M)} & \makecell{FLOPs\\(G)} & \makecell{mIoU\\(ss)} & \makecell{\miou\\(ms)} \\
Backbone & \#P.(M) & FLOPs(G) & mIoU(ss) & \miou(ms) \\
\midrule

\oursxt
    & 45 & 889 & 44.3 & 45.4 \\ % done
\midrule

Swin-T \cite{liu2021swin}
    & 60 & 945 & 44.5 & 45.8 \\ % github
Twins-S \cite{chu2021twins}
    & 54 & 931  & 46.2 & 47.1 \\
% & TwinsP-S \cite{chu2021twins}
%     & 55 & 983 & 46.2 / 47.5 \\
ConvNeXt-T \cite{liu2022convnext}
    & 60 & 939 & - & 46.7 \\
ASMLP-T \cite{lian2021asmlp}
    & 60 & 937 & - & 46.5 \\ % asmlp
CycleMLP-T \cite{chen2022cyclemlp}
    & 60 & 937 & - & 47.1 \\ % cycle
% & Shift-T \cite{wang2022shift}
%     & 60 & 942 & 46.3 & 47.8 \\
\ourst
    & 57 & 927 & \textbf{46.5} & \textbf{47.6} \\ % done
\bottomrule

Swin-S \cite{liu2021swin}
    & 81 & 1038 & 47.6 & 49.5 \\ % github
% & TwinsP-B \cite{chu2021twins}
%     & 74 & 1073 & 47.1 / 48.4 \\
Twins-B \cite{chu2021twins}
    & 89 & 1078 & 47.7 & 48.9 \\
ConvNeXt-S \cite{liu2022convnext}
    & 82 & 1027 & - & 49.6 \\
ASMLP-S \cite{lian2021asmlp}
    & 81 & 1024 & - & 49.2 \\ % asmlp
CycleMLP-S \cite{chen2022cyclemlp}
    & 81 & 1024 & - & 49.6 \\ % cycle
% & Shift-S \cite{wang2022shift}
%     & 81 & 1029 & 47.8 & 49.6 \\
\oursb
    & 82 & 1055 & \textbf{48.7} & \textbf{49.8} \\
\arrayrulecolor{black}\midrule

Swin-B \cite{liu2021swin}
    & 121 & 1188 & 48.1 & 49.7 \\ % github
% & TwinsP-L \cite{chu2021twins}
%     & 92 & 1179 & 48.6 / 49.8 \\
Twins-L \cite{chu2021twins}
    & 133 & 1236 & 48.8 & 50.2 \\
ConvNeXt-B \cite{liu2022convnext}
    & 122 & 1170 & - & 49.9 \\
ASMLP-B \cite{lian2021asmlp}
    & 121 & 1166 & - & 49.5 \\ % asmlp
CycleMLP-B \cite{chen2022cyclemlp}
    & 121 & 1166 & - & 49.7 \\ % cycle
% & Shift-B \cite{wang2022shift}
%     & 121 & 1174 & 47.9 & 49.2 \\
\ourss
    & 69 & 988 & 48.4 & 49.5 \\
\arrayrulecolor{white}\hline
\oursl
    & 108 & 1106 & \textbf{50.1} & \textbf{51.1} \\
\arrayrulecolor{black}\bottomrule
\end{NiceTabular}
}
\endgroup






% \begingroup

% \begin{tabular}{@{}c@{}}

% \begin{minipage}[b]{0.53\textwidth}
% \resizebox{\textwidth}{!}{
% \begin{NiceTabular}{@{}lcccc@{}}[code-before=
% \rectanglecolor{\rc}{8-1}{8-15}
% \rectanglecolor{\rc}{15-1}{16-15}
% ]
% \toprule
% Method & Backbone & \makecell{\#P.\\(M)} & \makecell{FLOPs\\(G)} & mIoU/mIoU(ms) \\
% \midrule

% UperNet \cite{xiao2018unifiedupernet}
%     & ResNet101 & 86 & 1029 & 43.8 / 44.9 \\
% % OCRNet \cite{yuan2020OCRNet}
% %     & HRNet-w48 & 71 & 664 & - & 45.7 \\
% ACNet \cite{fu2019ACNet}
%     & ResNet101 & 69 & 1119 & - & 45.9 \\
% DNL \cite{yin2020DNL}
%     & ResNet101 & 69 & 1249 & - & 46.0 \\
% % DLabV3+ \cite{chen2018DeepLabv3plus}
% %     & ResNeSt-101 & 66 & 1051 & 46.5 & 47.3 \\
% DLabV3+ \cite{chen2018DeepLabv3plus}
%     & ResNeSt-200 & 88 & 1381 & - & 48.4 \\

% % SETR-PUP \cite{zheng2021SETR}
% %     & ViT-L$\ddagger$   & 310 & \multicolumn{1}{c}{-} & 48.6 / 50.1 \\
% SETR-MLA \cite{zheng2021SETR}
%     & ViT-L$\ddagger$   & 308 & \multicolumn{1}{c}{-} & 48.6 / 50.3 \\
% \midrule

% UperNet \cite{xiao2018unifiedupernet}
% & \oursxt
%     & 45 & 889 & 44.3 / 45.4 \\ % done
% \midrule

% \multirow{6}{*}{UperNet \cite{xiao2018unifiedupernet}}
% & Swin-T \cite{liu2021swin}
%     & 60 & 945 & 44.5 / 45.8 \\ % github
% & Twins-S \cite{chu2021twins}
%     & 54 & 931  & 46.2 / 47.1 \\
% % & TwinsP-S \cite{chu2021twins}
% %     & 55 & 983 & 46.2 / 47.5 \\
% & ConvNeXt-T \cite{liu2022convnext}
%     & 60 & 939 & - & 46.7 \\
% & ASMLP-T \cite{lian2021asmlp}
%     & 60 & 937 & - & 46.5 \\ % asmlp
% & CycleMLP-T \cite{chen2022cyclemlp}
%     & 60 & 937 & - & 47.1 \\ % cycle
% % & Shift-T \cite{wang2022shift}
% %     & 60 & 942 & 46.3 & 47.8 \\
% & \ourst
%     & 57 & 927 & \textbf{46.5} / \textbf{47.6} \\ % done
% \bottomrule


% \end{NiceTabular}
% }
% \end{minipage}


% \begin{minipage}[b]{0.455\textwidth}
% \resizebox{\textwidth}{!}{
% \begin{NiceTabular}{@{}ccccc@{}}[code-before=
% \rectanglecolor{\rc}{8-1}{8-15}
% \rectanglecolor{\rc}{15-1}{16-15}
% ]
% \toprule
% Method & Backbone & \makecell{\#P.\\(M)} & \makecell{FLOPs\\(G)} & mIoU/mIoU(ms) \\
% \midrule

% \multirow{8}{*}{\rotatebox{270}{UperNet \cite{xiao2018unifiedupernet}}}
% & Swin-S \cite{liu2021swin}
%     & 81 & 1038 & 47.6 / 49.5 \\ % github
% % & TwinsP-B \cite{chu2021twins}
% %     & 74 & 1073 & 47.1 / 48.4 \\
% & Twins-B \cite{chu2021twins}
%     & 89 & 1078 & 47.7 / 48.9 \\
% & ConvNeXt-T \cite{liu2022convnext}
%     & 82 & 1027 & - & 49.6 \\
% & ASMLP-S \cite{lian2021asmlp}
%     & 81 & 1024 & - & 49.2 \\ % asmlp
% & CycleMLP-S \cite{chen2022cyclemlp}
%     & 81 & 1024 & - & 49.6 \\ % cycle
% % & Shift-S \cite{wang2022shift}
% %     & 81 & 1029 & 47.8 & 49.6 \\
% & \ourss
%     & 69 & 988 & 48.4 / 49.5 \\
% \arrayrulecolor{white}\hline
% &  \oursb
%     & 82 & 1055 & \textbf{48.7} / \textbf{49.8} \\
% \arrayrulecolor{black}\midrule

% \multirow{7}{*}{\rotatebox{270}{UperNet \cite{xiao2018unifiedupernet}}}
% & Swin-B \cite{liu2021swin}
%     & 121 & 1188 & 48.1 / 49.7 \\ % github
% % & TwinsP-L \cite{chu2021twins}
% %     & 92 & 1179 & 48.6 / 49.8 \\
% & Twins-L \cite{chu2021twins}
%     & 133 & 1236 & 48.8 / 50.2 \\
% & ConvNeXt-T \cite{liu2022convnext}
%     & 122 & 1170 & - & 49.9 \\
% & ASMLP-B \cite{lian2021asmlp}
%     & 121 & 1166 & - & 49.5 \\ % asmlp
% & CycleMLP-B \cite{chen2022cyclemlp}
%     & 121 & 1166 & - & 49.7 \\ % cycle
% % & Shift-B \cite{wang2022shift}
% %     & 121 & 1174 & 47.9 & 49.2 \\
% & \oursl
%     & 108 & 1106 & \textbf{50.1} / \textbf{51.1} \\
% \bottomrule
% \end{NiceTabular}
% }
% \end{minipage}
% \end{tabular}
% \endgroup





==> tables/ade_20k_back.tex <==
\begingroup

\resizebox{0.5\textwidth}{!}{    
\begin{NiceTabular}{l@{}|c|cc|cc}
\CodeBefore 
\rectanglecolor{\rc}{4-2}{4-}
\rectanglecolor{\rc}{12-2}{12-}
\rectanglecolor{\rc}{20-2}{21-}
\rectanglecolor{\rc}{29-2}{29-}
\Body
\hline
Method & Backbone & \#P.(M) & GFLOPs & mIoU~ & ~MS mIoU \\
\hline

ACNet \cite{fu2019ACNet}
    & ResNet101 & 69 & 1119 & - & 45.9 \\
UperNet \cite{xiao2018unifiedupernet}
    & ResNet101 & 86 & 1029 & 43.8 & 44.9 \\
DNL \cite{yin2020DNL}
    & ResNet101 & 69 & 1249 & - & 46.0 \\
OCRNet \cite{yuan2020OCRNet}
    & HRNet-w48 & 71 & 664 & - & 45.7 \\
DeepLabV3+ \cite{chen2018DeepLabv3plus}
    & ResNeSt-200 & 88 & 1381 & - & 48.4 \\
\hline

SETR-PUP \cite{zheng2021SETR}
    & ViT-L$\ddagger$   & 310 & - & 48.6 & 50.1 \\
SETR-MLA \cite{zheng2021SETR}
    & ViT-L$\ddagger$   & 308 & - & 48.6 & 50.3 \\
\hline

UperNet \cite{xiao2018unifiedupernet}
& \oursxt
    & 45.3 & 889 & 44.3 & 45.4 \\ % done
\hline


\multirow{6}{*}{UperNet \cite{xiao2018unifiedupernet}}
& Swin-T \cite{liu2021swin}
    & 59.9 & 945 & 44.5 & 45.8 \\ % github
& Twins-S \cite{chu2021twins}
    & 54.4 & -  & 46.2 & 47.1 \\ 
& TwinsP-S \cite{chu2021twins}
    & 54.6 & - & 46.2 & 47.5 \\
& ASMLP-T \cite{lian2021asmlp}
    & 60 & 937 & - & 46.5 \\ % asmlp
& CycleMLP-T \cite{chen2022cyclemlp} 
    & 60 & 937 & - & 47.1 \\ % cycle 
& Shift-T \cite{wang2022shift}
    & 60 & 942 & 46.3 & 47.8 \\
& ConvNeXt-T \cite{liu2022convnext}
    & 60 & 939 & - & 46.7 \\
& \ourst
    & 57.1 & 927 & \textbf{46.5} & \textbf{47.6} \\ % done
\hline

\multirow{1}{*}{UperNet \cite{xiao2018unifiedupernet}}
& Swin-S \cite{liu2021swin}
    & 81 & 1038 & 47.6 & 49.5 \\ % github
& Twins-B \cite{chu2021twins}
    & 88.5 & -  & 47.7 & 48.9 \\ 
& TwinsP-B \cite{chu2021twins}
    & 74.3 & - & 47.1 & 48.4 \\
& ASMLP-S \cite{lian2021asmlp}
    & 81 & 1024 & - & 49.2 \\ % asmlp
& CycleMLP-S \cite{chen2022cyclemlp} 
    & 81 & 1024 & - & 49.6 \\ % cycle 
& Shift-S \cite{wang2022shift}
    & 81 & 1029 & 47.8 & 49.6 \\
& ConvNeXt-T \cite{liu2022convnext}
    & 82 & 1027 & - & 49.6 \\
& \ourss
    & 68.6 & 988 & 48.4 & 49.5 \\
\arrayrulecolor{white}\hline
&  \oursb
    & 82.1 & 1055 & \textbf{48.7} & \textbf{49.8} \\
\arrayrulecolor{black}\hline


\multirow{1}{*}{UperNet \cite{xiao2018unifiedupernet}}
& Swin-B \cite{liu2021swin}
    & 121 & 1188 & 48.1 & 49.7 \\ % github
& Twins-L \cite{chu2021twins}
    & 133 & -  & 48.8 & 50.2 \\ 
& TwinsP-L \cite{chu2021twins}
    & 91.5 & - & 48.6 & 49.8 \\
& ASMLP-B \cite{lian2021asmlp}
    & 121 & 1166 & - & 49.5 \\ % asmlp
& CycleMLP-B \cite{chen2022cyclemlp} 
    & 121 & 1166 & - & 49.7 \\ % cycle 
& Shift-B \cite{wang2022shift}
    & 121 & 1174 & 47.9 & 49.2 \\
& ConvNeXt-T \cite{liu2022convnext}
    & 122 & 1170 & - & 49.9 \\
& \oursl
    & 107.9 & 1106 & \textbf{50.1} & \textbf{51.1} \\
\hline

\end{NiceTabular}
}

\endgroup

==> tables/ade_back_aaai.tex <==
\begingroup
\footnotesize
\begin{tabular}{@{}>{\columncolor{white}[0pt][\tabcolsep]}c@{}}


\begin{minipage}{0.33\linewidth}
% \resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{NiceTabular}{@{}lccc@{}}[code-before=
\rectanglecolor{\rc}{8-1}{8-5}
\rectanglecolor{\rc}{14-1}{15-5}
]
\toprule
\multicolumn{4}{c}{UperNet} \\
Model & \#P & FLOPs & mIoU/mIoU(ms)  \\

\midrule
% Resnet50      & 67    & 953   & 42.6 / 43.5 \\     
Swin-T       & 60    & 945   & 44.5 / 45.8 \\ % github
Twins-S      & 54    & 931   & 46.2 / 47.1 \\
% TwinsP-S     & 55    & 983   & 46.2 / 47.5 \\
ConvNeXt-T    & 60    & 939   & \quad-\phantom{..}/ 46.7 \\
ASMLP-T       & 60    & 937   & \quad-\phantom{..}/ 46.5 \\ % asmlp
CycleMLP-T    & 60    & 937   & \quad-\phantom{..}/ 47.1 \\ % cycle
%Shift-T  & 60 & 942 & 46.3/ 47.8 \\
\ourst        & 57    & 927   & \textbf{46.5 / 47.6} \\ 

\midrule
% ResNet101     & 86    & 1029  & 43.8 / 44.9 \\
Swin-B       & 121   & 1188  & 48.1 / 49.7 \\ % github
% TwinsP-L     & 92    & 1179  & 48.6 / 49.8 \\
Twins-L      & 133   & 1236  & 48.8 / 50.2 \\
ConvNeXt-T    & 122   & 1170  & \quad-\phantom{..}/ 49.9 \\
ASMLP-B       & 121   & 1166  & \quad-\phantom{..}/ 49.5 \\ % asmlp
CycleMLP-B    & 121   & 1166  & \quad-\phantom{..}/ 49.7 \\ % cycle
% Shift-B    & 121 & 1174 & 47.9/ 49.2 \\
\ourss        & 69    & 988  & 48.4 / 49.5 \\
\arrayrulecolor{white}\hline
\oursl        & 108   & 1106  & \textbf{50.1 / 51.1} \\
\arrayrulecolor{black}\bottomrule
\end{NiceTabular}
\captionof{table}{Semantic segmentation results on ADE20K \texttt{val} with UperNet. FLOPs are evaluated on 512$\times$2048. mIoU(ms): mIoU with multi-scale inference.}
\label{table: upernet}
\end{minipage}

\hspace{0.01\textwidth}


\begin{minipage}{0.3\linewidth}
% \resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}lccc@{}}[code-before=
\rectanglecolor{\rc}{9-1}{9-5}
\rectanglecolor{\rc}{15-1}{15-5}
]
\toprule
\multicolumn{4}{c}{Semantic FPN} \\
Model & \#P & FLOPs & mIoU  \\


% \hline
% ResNet18      & 15.5  & 32    & 32.9 \\  % pvt
% PVT-T        & 17.0  & 33    & 35.7 \\
% P2T-T        & 14.9  & 32    & 39.5 \\
% CycleMLP-B1   & 18.9  & 33    & 40.8 \\
% WaveMLP-T     & 19.3  & -     & 41.2 \\
% \oursxt       & 19.1  & 33.1 & \textbf{43.0} \\


\midrule
% ResNet50      & 28.5  & 46    & 36.7 \\  % pvt
% PVT-S        & 28.2  & 45    & 39.8 \\
Swin-T       & 31.9  & 48    & 41.5 \\
Twins-S      & 28.3  & 37    & 43.2 \\
TwinsP-S     & 28.4  & 40    & 44.3 \\
% P2T-S        & 26.8  & 42    & 44.4 \\
% GFNet-T     & FFT   & 26.6  & -     & 41.0 \\
MorphMLP-T    & 26.4  & -     & 43.0 \\
CycleMLP-B2   & 30.6  & 42    & 43.4 \\ 
Wave-MLP-S    & 31.2  & -     & 44.4 \\
\ourst        & 30.9  & 42.4  & \textbf{45.8} \\
\midrule
% ResNeXt101    & 86.4  & 104   & 40.2 \\
% PVT-L        & 65.1  & 80    & 42.1 \\
Swin-B       & 91.2  & 107   & 46.0 \\ % twins
TwinsP-L     & 65.3  & 71    & 46.4 \\
Twins-L      & 103.7 & 102   & 46.7 \\
% GFNet \cite{rao2021GFNet}
%     & FFT   & 74.7 & - & 44.8 \\
CycleMLP-B5   & 79.4  & 86    & 45.5 \\
MorphMLP-B    & 59.3  & -     & 45.9 \\
% \oursb        & 55.9  & 74.7  & \textbf{47.7} \\
\arrayrulecolor{white}\hline
\oursl        & 79.8  & 86.6  &\textbf{48.1} \\
\arrayrulecolor{black}\bottomrule

\end{NiceTabular}
\captionof{table}{Semantic segmentation results on ADE20K \texttt{val} with Semantic FPN. FLOPs are evaluated on 512$\times$512. }
\label{table: semantic-fpn}
\end{minipage}

\hspace{0.01\textwidth}

\begin{minipage}{0.3\linewidth}
\resizebox{\textwidth}{!}{
\includegraphics[width=\linewidth]{images/bubble_fpn.png}
}
\captionof{figure}{Comparisons of mIoU and the FLOPs for Semantic FPN. Bubble size corresponds to the model size.}
\label{fig: semantic-fpn}
\end{minipage}


\end{tabular}
\endgroup



==> tables/ade_fpn.tex <==
\begingroup
\small
\setlength{\tabcolsep}{11pt}
% \resizebox{0.475\textwidth}{!}{ 
\begin{NiceTabular}{@{}lccc@{}}[code-before=
\rectanglecolor{\rc}{4-1}{4-15}
\rectanglecolor{\rc}{10-1}{10-15}
\rectanglecolor{\rc}{15-1}{15-15}
\rectanglecolor{\rc}{20-1}{21-15}
]
\toprule
Backbone & \#P.(M) & FLOPs(G) & mIoU(ss)  \\

\midrule
% ResNet18 \cite{he2016deepresnet}
%     & 15.5 & 32.2 & 32.9 \\  % pvt
% PVT-T \cite{wang2021pyramidpvt} 
%     & 17.0 & 33.2 & 35.7 \\
% P2T-T \cite{wu2021p2t}
%     & 14.9 & 31.8 & 39.5 \\
CycleMLP-B1 \cite{chen2022cyclemlp}
    & 18.9 & 32.8 & 40.8 \\
WaveMLP-T \cite{tang2021imagewavemlp}
    & 19.3 & - & 41.2 \\
\oursxt
    & 19.1 & 33.1 & \textbf{43.0} \\
\midrule


% ResNet50 \cite{he2016deepresnet} 
%     & 28.5 & 45.6  & 36.7 \\  % pvt
Swin-T \cite{liu2021swin}  % twins
    & 31.9 & 46 & 41.5 \\
% PVT-S \cite{wang2021pyramidpvt} 
%     & 28.2 & 44.5 & 39.8 \\
% P2T-S \cite{wu2021p2t}  
%     & 26.8 & 41.7 & 44.4 \\
Twins-S \cite{chu2021twins}
    & 28.3 & 37 & 43.2 \\
% TwinsP-S \cite{chu2021twins}
%     & 28.4 & 40 & 44.3 \\
% GFNet-T \cite{rao2021GFNet}
%     & 26.6 & - & 41.0 \\
MorphMLP-T \cite{zhang2021morphmlp}
    & 26.4 & - & 43.0 \\
CycleMLP-B2 \cite{chen2022cyclemlp}
    & 30.6 & 42.0 & 43.4 \\ 
Wave-MLP-S \cite{tang2021imagewavemlp}  
    & 31.2 & - & 44.4 \\
\ourst
    & 30.9 & 42.4 & \textbf{45.8} \\
\midrule

% ResNet101 \cite{he2016deepresnet}
%     & 47.5 & 65.1 & 38.8 \\
% ResNeXt101-32$\times$4d \cite{xie2017ResNeXt}
%      & 47.1 & 64.7 & 39.7 \\
% PVT-M \cite{wang2021pyramidpvt}
%     & 48.0 & 61.0 & 41.6 \\
% P2T-B \cite{wu2021p2t}
%      & 39.9 & 57.5 & 46.2 \\
Swin-S \cite{liu2021swin} 
    & 53.2 & 70 & 45.2 \\
% TwinsP-B \cite{chu2021twins}
%     & 48.1 & 55 & 44.9 \\
Twins-B \cite{chu2021twins}
    & 60.4 & 67 & 45.3 \\
% GFNet-S \cite{rao2021GFNet}
%     & FFT   & 47.5 & - & 42.5 \\ 
CycleMLP-B3 \cite{chen2022cyclemlp}
    & 42.1 & 57.5 & 44.3 \\
% CycleMLP-B4 \cite{chen2022cyclemlp}
%        & 55.6 & - & 45.1 \\
WaveMLP-M \cite{tang2021imagewavemlp}
    & 43.3 & - & 46.8 \\
\ourss 
    & 42.4 & 57.8 & \textbf{47.3} \\
\midrule


% ResNeXt101 \cite{xie2017ResNeXt}
%     &  86.4 & 103.9 & 40.2 \\
% PVT-L \cite{wang2021pyramidpvt} 
%     & 65.1 & 79.6 & 42.1 \\
% TwinsP-L \cite{chu2021twins}
    % & 65.3 & 71 & 46.4 \\
Swin-B \cite{liu2021swin}
    & 91.2 & 107 & 46.0 \\ % twins
Twins-L \cite{chu2021twins}
    & 103.7 & 102 & 46.7 \\
% GFNet \cite{rao2021GFNet}
%     & FFT   & 74.7 & - & 44.8 \\
MorphMLP-B \cite{zhang2021morphmlp}
    & 59.3 & - & 45.9 \\
CycleMLP-B5 \cite{chen2022cyclemlp}
    & 79.4 & 86.0 & 45.5 \\
\oursb
    & 55.9 & 74.7 & 47.7 \\
\arrayrulecolor{white}\hline
\oursl
    & 79.8 & 86.6 &\textbf{48.1} \\
\arrayrulecolor{black}\bottomrule
\end{NiceTabular}
% }
\endgroup








% \begingroup
% \small

% \begin{tabular}{@{}c@{}}

% \hspace{0.05\textwidth}
% % ========================================= left
% \begin{minipage}{0.45\linewidth}
% % \resizebox{\textwidth}{!}{ 
% \begin{NiceTabular}{@{}lccc@{}}[code-before=
% \rectanglecolor{\rc}{6-1}{6-15}
% \rectanglecolor{\rc}{16-1}{16-15}
% ]
% \toprule
% Backbone & \#P.(M) & FLOPs(G) & mIoU  \\
% % =============== FLOPs: 512x512


% \midrule
% ResNet18 \cite{he2016deepresnet}
%     & 15.5 & 32.2 & 32.9 \\  % pvt
% % PVT-T \cite{wang2021pyramidpvt} 
% %     & 17.0 & 33.2 & 35.7 \\
% P2T-T \cite{wu2021p2t}
%     & 14.9 & 31.8 & 39.5 \\
% CycleMLP-B1 \cite{chen2022cyclemlp}
%     & 18.9 & 32.8 & 40.8 \\
% WaveMLP-T \cite{tang2021imagewavemlp}
%     & 19.3 & - & 41.2 \\
% \oursxt
%     & 19.1 & 33.1 & \textbf{43.0} \\
% \midrule


% ResNet50 \cite{he2016deepresnet} 
%     & 28.5 & 45.6  & 36.7 \\  % pvt
% Swin-T \cite{liu2021swin}  % twins
%     & 31.9 & 46 & 41.5 \\
% % PVT-S \cite{wang2021pyramidpvt} 
% %     & 28.2 & 44.5 & 39.8 \\
% P2T-S \cite{wu2021p2t}  
%     & 26.8 & 41.7 & 44.4 \\
% Twins-S \cite{chu2021twins}
%     & 28.3 & 37 & 43.2 \\
% TwinsP-S \cite{chu2021twins}
%     & 28.4 & 40 & 44.3 \\
% GFNet-T \cite{rao2021GFNet}
%     & 26.6 & - & 41.0 \\
% MorphMLP-T \cite{zhang2021morphmlp}
%     & 26.4 & - & 43.0 \\
% CycleMLP-B2 \cite{chen2022cyclemlp}
%     & 30.6 & 42.0 & 43.4 \\ 
% Wave-MLP-S \cite{tang2021imagewavemlp}  
%     & 31.2 & - & 44.4 \\
% \ourst
%     & 30.9 & 42.4 & \textbf{45.8} \\
% \bottomrule

% \end{NiceTabular}
% % }
% \end{minipage}

% \hspace{0.05\textwidth}

% %  ============================================== right
% \begin{minipage}{0.45\linewidth}
% % \resizebox{\textwidth}{!}{    
% \begin{NiceTabular}{@{}lccc@{}}[code-before=
% \rectanglecolor{\rc}{8-1}{8-15}
% \rectanglecolor{\rc}{15-1}{16-15}
% ]
% \toprule
% Backbone & \#P.(M) & FLOPs(G) & mIoU  \\


% \midrule
% ResNet101 \cite{he2016deepresnet}
%     & 47.5 & 65.1 & 38.8 \\
% % ResNeXt101-32$\times$4d \cite{xie2017ResNeXt}
% %      & 47.1 & 64.7 & 39.7 \\
% % PVT-M \cite{wang2021pyramidpvt}
% %     & 48.0 & 61.0 & 41.6 \\
% % P2T-B \cite{wu2021p2t}
% %      & 39.9 & 57.5 & 46.2 \\
% Swin-S \cite{liu2021swin} 
%     & 53.2 & 70 & 45.2 \\
% TwinsP-B \cite{chu2021twins}
%     & 48.1 & 55 & 44.9 \\
% Twins-B \cite{chu2021twins}
%     & 60.4 & 67 & 45.3 \\
% % GFNet-S \cite{rao2021GFNet}
% %     & FFT   & 47.5 & - & 42.5 \\ 
% CycleMLP-B3 \cite{chen2022cyclemlp}
%     & 42.1 & 57.5 & 44.3 \\
% % CycleMLP-B4 \cite{chen2022cyclemlp}
% %        & 55.6 & - & 45.1 \\
% WaveMLP-M \cite{tang2021imagewavemlp}
%     & 43.3 & - & 46.8 \\
% \ourss 
%     & 42.4 & 57.8 & \textbf{47.3} \\
% \midrule


% ResNeXt101 \cite{xie2017ResNeXt}
%     &  86.4 & 103.9 & 40.2 \\
% % PVT-L \cite{wang2021pyramidpvt} 
% %     & 65.1 & 79.6 & 42.1 \\
% TwinsP-L \cite{chu2021twins}
%     & 65.3 & 71 & 46.4 \\
% Swin-B \cite{liu2021swin}
%     & 91.2 & 107 & 46.0 \\ % twins
% Twins-L \cite{chu2021twins}
%     & 103.7 & 102 & 46.7 \\
% % GFNet \cite{rao2021GFNet}
% %     & FFT   & 74.7 & - & 44.8 \\
% MorphMLP-B \cite{zhang2021morphmlp}
%     & 59.3 & - & 45.9 \\
% CycleMLP-B5 \cite{chen2022cyclemlp}
%     & 79.4 & 86.0 & 45.5 \\
% \oursb
%     & 55.9 & 74.7 & 47.7 \\
% \arrayrulecolor{white}\hline
% \oursl
%     & 79.8 & 86.6 &\textbf{48.1} \\
% \arrayrulecolor{black}\bottomrule
% \end{NiceTabular}
% % }
% \end{minipage}

% \end{tabular}

% \endgroup

==> tables/ade_fpn_back.tex <==
\begingroup
% \scriptsize

\begin{tabular}{@{}>{\columncolor{white}[0pt][\tabcolsep]}c@{}}

% ========================================= left
\begin{minipage}{0.48\linewidth}
\resizebox{\textwidth}{!}{ 
\begin{NiceTabular}{l@{}|c|cc|c}
% \toprule
\hline
Model & Arch. & \#P.(M) & GFLOPs & mIoU  \\
% =============== FLOPs: 512x512


\hline
ResNet18 \cite{he2016deepresnet}
    & CNN   & 15.5 & 32.2 & 32.9 \\  % pvt
PVT-T \cite{wang2021pyramidpvt} 
    & Trans & 17.0 & 33.2 & 35.7 \\
P2T-T \cite{wu2021p2t}
    & Trans & 14.9 & 31.8 & 39.5 \\
CycleMLP-B1 \cite{chen2022cyclemlp}
    & MLP   & 18.9 & 32.8 & 40.8 \\
WaveMLP-T \cite{tang2021imagewavemlp}
    & MLP   & 19.3 & - & 41.2 \\
\rowcolor{Gray!25}\oursxt
    & MLP   & 19.1 & 33.1 & \textbf{43.0} \\
\hline


ResNet50 \cite{he2016deepresnet} 
    & CNN   & 28.5 & 45.6  & 36.7 \\  % pvt
Swin-T \cite{liu2021swin}  % twins
    & Trans & 31.9 & 46 & 41.5 \\
PVT-S \cite{wang2021pyramidpvt} 
    & Trans & 28.2 & 44.5 & 39.8 \\
P2T-S \cite{wu2021p2t}
    & Trans & 26.8 & 41.7 & 44.4 \\
Twins-S \cite{chu2021twins}
    & Trans & 28.3 & 37 & 43.2 \\
TwinsP-S \cite{chu2021twins}
    & Trans & 28.4 & 40 & 44.3 \\
GFNet-T \cite{rao2021GFNet}
    & FFT   & 26.6 & - & 41.0 \\
MorphMLP-T \cite{zhang2021morphmlp}
    & MLP   & 26.4 & - & 43.0 \\
CycleMLP-B2 \cite{chen2022cyclemlp}
    & MLP & 30.6 & 42.0 & 43.4 \\ 
Wave-MLP-S \cite{tang2021imagewavemlp}  
    & MLP & 31.2 & - & 44.4 \\
\rowcolor{\rc}\ourst
    & MLP   & 30.9 & 42.4 & \textbf{45.8} \\
\hline

% ResNet101 \cite{he2016deepresnet}
%     & CNN & 47.5 & 65.1 & 38.8 \\
% % ResNeXt101-32$\times$4d \cite{xie2017ResNeXt}
% %     & CNN & 47.1 & 64.7 & 39.7 \\
% PVT-M \cite{wang2021pyramidpvt}
%     & Trans & 48.0 & 61.0 & 41.6 \\
% P2T-B \cite{wu2021p2t}
%     & Trans & 39.9 & 57.5 & 46.2 \\
% Swin-S \cite{liu2021swin} 
%     & Trans & 53.2 & 70 & 45.2 \\
% TwinsP-B \cite{chu2021twins}
%     & Trans & 48.1 & 55 & 44.9 \\
% Twins-B \cite{chu2021twins}
%     & Trans & 60.4 & 67 & 45.3 \\
% GFNet-S \cite{rao2021GFNet}
%     & FFT   & 47.5 & - & 42.5 \\ 
% CycleMLP-B3 \cite{chen2022cyclemlp}
%     & MLP   & 42.1 & - & 44.3 \\
% CycleMLP-B4 \cite{chen2022cyclemlp}
%     & MLP   & 55.6 & - & 45.1 \\
% WaveMLP-M \cite{tang2021imagewavemlp}
%     & MLP   & 43.3 & - & 46.8 \\
% \rowcolor{\rc}
% \ourss 
%     & MLP   & - & - & 47.3 \\
% \hline


% % ResNeXt101-64$\times$4d \cite{xie2017ResNeXt}
% %     & CNN &  86.4 & 103.9 & 40.2 \\
% PVT-L \cite{wang2021pyramidpvt} 
%     & Trans & 65.1 & 79.6 & 42.1 \\
% TwinsP-L \cite{chu2021twins}
%     & Trans & 65.3 & 71 & 46.4 \\
% Swin-B \cite{liu2021swin}
%     & Trans & 91.2 & 107 & 46.0 \\ % twins
% Twins-L \cite{chu2021twins}
%     & Trans & 103.7 & 102 & 46.7 \\
% GFNet \cite{rao2021GFNet}
%     & FFT   & 74.7 & - & 44.8 \\
% CycleMLP-B5 \cite{chen2022cyclemlp}
%     & MLP   & 79.4 & - & 45.5 \\
% \rowcolor{\rc}\oursb
%     & MLP   & - & - & 47.7 \\
% \arrayrulecolor{white}\hline
% \rowcolor{\rc}\oursl
%     & MLP   & - & - & 48.1 \\

% \arrayrulecolor{black}\hline
\end{NiceTabular}
		}
\end{minipage}

%  ============================================== right
\begin{minipage}{0.48\linewidth}
\resizebox{\textwidth}{!}{    
\begin{NiceTabular}{l@{}|c|cc|c}
% \toprule
\hline
Model & Arch. & \#P.(M) & GFLOPs & mIoU  \\
% =============== FLOPs: 512x512


\hline
% ResNet18 \cite{he2016deepresnet}
%     & CNN   & 15.5 & 32.2 & 32.9 \\  % pvt
% PVT-T \cite{wang2021pyramidpvt} 
%     & Trans & 17.0 & 33.2 & 35.7 \\
% P2T-T \cite{wu2021p2t}
%     & Trans & 14.9 & 31.8 & 39.5 \\
% CycleMLP-B1 \cite{chen2022cyclemlp}
%     & MLP   & 18.9 & - & 40.8 \\
% WaveMLP-T \cite{tang2021imagewavemlp}
%     & MLP   & 19.3 & - & 41.2 \\
% \rowcolor{Gray!25}\oursxt
%     & MLP   & - & - & 43.0 \\
% \hline


% ResNet50 \cite{he2016deepresnet} 
%     & CNN   & 28.5 & 45.6  & 36.7 \\  % pvt
% Swin-T \cite{liu2021swin}  % twins
%     & Trans & 31.9 & 46 & 41.5 \\
% PVT-S \cite{wang2021pyramidpvt} 
%     & Trans & 28.2 & 44.5 & 39.8 \\
% P2T-S \cite{wu2021p2t}
%     & Trans & 26.8 & 41.7 & 44.4 \\
% Twins-S \cite{chu2021twins}
%     & Trans & 28.3 & 37 & 43.2 \\
% TwinsP-S \cite{chu2021twins}
%     & Trans & 28.4 & 40 & 44.3 \\
% GFNet-T \cite{rao2021GFNet}
%     & FFT   & 26.6 & - & 41.0 \\
% CycleMLP-T \cite{chen2022cyclemlp}
%     & MLP & 30.6 & - & 43.4 \\ 
% Wave-MLP-S \cite{tang2021imagewavemlp}  
%     & MLP & 31.2 & - & 44.4 \\
% \rowcolor{\rc}\ourst
%     & MLP   & & & 45.8 \\
% \hline

ResNet101 \cite{he2016deepresnet}
    & CNN & 47.5 & 65.1 & 38.8 \\
% ResNeXt101-32$\times$4d \cite{xie2017ResNeXt}
%     & CNN & 47.1 & 64.7 & 39.7 \\
PVT-M \cite{wang2021pyramidpvt}
    & Trans & 48.0 & 61.0 & 41.6 \\
% P2T-B \cite{wu2021p2t}
%     & Trans & 39.9 & 57.5 & 46.2 \\
Swin-S \cite{liu2021swin} 
    & Trans & 53.2 & 70 & 45.2 \\
TwinsP-B \cite{chu2021twins}
    & Trans & 48.1 & 55 & 44.9 \\
Twins-B \cite{chu2021twins}
    & Trans & 60.4 & 67 & 45.3 \\
% GFNet-S \cite{rao2021GFNet}
%     & FFT   & 47.5 & - & 42.5 \\ 
CycleMLP-B3 \cite{chen2022cyclemlp}
    & MLP   & 42.1 & 57.5 & 44.3 \\
% CycleMLP-B4 \cite{chen2022cyclemlp}
%     & MLP   & 55.6 & - & 45.1 \\
WaveMLP-M \cite{tang2021imagewavemlp}
    & MLP   & 43.3 & - & 46.8 \\
\rowcolor{\rc}
\ourss 
    & MLP   & 42.4 & 57.8 & 47.3 \\
\hline


ResNeXt101 \cite{xie2017ResNeXt}
    & CNN &  86.4 & 103.9 & 40.2 \\
PVT-L \cite{wang2021pyramidpvt} 
    & Trans & 65.1 & 79.6 & 42.1 \\
TwinsP-L \cite{chu2021twins}
    & Trans & 65.3 & 71 & 46.4 \\
Swin-B \cite{liu2021swin}
    & Trans & 91.2 & 107 & 46.0 \\ % twins
Twins-L \cite{chu2021twins}
    & Trans & 103.7 & 102 & 46.7 \\
% GFNet \cite{rao2021GFNet}
%     & FFT   & 74.7 & - & 44.8 \\
MorphMLP-B \cite{zhang2021morphmlp}
    & MLP   & 59.3 & - & 45.9 \\
CycleMLP-B5 \cite{chen2022cyclemlp}
    & MLP   & 79.4 & 86.0 & 45.5 \\
\rowcolor{\rc}\oursb
    & MLP   & 55.9 & 74.7 & \textbf{47.7} \\
\arrayrulecolor{white}\hline
\rowcolor{\rc}\oursl
    & MLP   & 79.8 & 86.6 &\textbf{48.1} \\

\arrayrulecolor{black}\hline
\end{NiceTabular}
}
\end{minipage}

\end{tabular}

\endgroup

==> tables/arch_list.tex <==
\begingroup

\setlength{\tabcolsep}{4pt}
\begin{NiceTabular}{@{}l|c|c|c|c|c@{}}

\hline
  & xTiny & Tiny & Small & Base & Large \\
\hline
\#P
    & 15.4M
    & 27.2M
    & 38.6M
    & 51.9M
    & 76.4M \\
\hline
FLOPs   
    & 2.2G 
    & 4.0G  
    & 6.9G  
    & 10.1G  
    & 12.3G \\
\hline
INT
    & 79.7
    & 82.0
    & 83.1 
    & 83.5
    & 83.8 \\   
\hline
COCO
    & 42.9/39.3 
    & 45.8/41.6 
    & 46.8/42.5 
    & 47.0/42.7 
    & 47.4/43.0 \\
\hline
\end{NiceTabular}
% 		}
\vspace{-0.3cm}
\endgroup

==> tables/coco_cascade_all.tex <==
\small
% \resizebox{\textwidth}{!}{    
\begin{NiceTabular}{@{}lcccccccccccccc@{}}[code-before=
\rectanglecolor{\rc}{8-1}{9-15}
\rectanglecolor{\rc}{13-1}{15-15}
]
\toprule
\multirow{2}{*}{Backbone} & \Block{2-1}{\makecell{\#Params.\\(M)}} & \multirow{2}{*}{\makecell{FLOPs\\{(G)}}} & \multicolumn{6}{c}{\normalsize Cascade Mask R-CNN 1$\times$} & \multicolumn{6}{c}{\normalsize Cascade Mask R-CNN 3$\times$ MS} \\
& & & \textbf{AP$^b$} & AP$^b_{50}$ & AP$^b_{75}$ & \textbf{AP$^m$} & AP$^m_{50}$ & AP$^m_{75}$ & \textbf{AP$^b$} & AP$^b_{50}$ & AP$^b_{75}$ & \textbf{AP$^m$} & AP$^m_{50}$ & AP$^m_{75}$ \\

\midrule

% ResNet-50 \cite{he2016deepresnet} & 82 & 739 
%     &- &- &- &- &- &-
%     & 46.3 & 64.3 & 50.5 & 40.1 & 61.7 & 43.4 \\ % cswin
Deit-S \cite{touvron2021deit} & 80 & 889 
    &- &- &- &- &- &-
    & 48.0 & 67.2 & 51.7 & 41.4 & 64.2 & 44.3 \\ %asmlp
Swin-T \cite{liu2021swin} & 86 & 745
    & 48.1 & 67.1 & 52.2 & 41.7 & 64.4 & 45.0
    & 50.4 & 69.2 & 54.7 & 43.7 & 66.6 & 47.3 \\ % github
ConvNeXt-T \cite{liu2022convnext} & 86 & 741 
    &- &- &- &- &- &-
    & 50.4 & 69.1 & 54.8 & 43.7 & 66.5 & 47.3 \\
% PVTv2-B2-Li \cite{wang2021pvtv2} & 80 & 725
%     &- &- &- &- &- &-
%     & 50.9 & 69.5 & 55.2 & -& -& -\\ % pvtv2
% PVTv2-B2 \cite{wang2021pvtv2} & 83 & 788
%     &- &- &- &- &- &-
%     & 51.1 & 69.8 & 55.3 & -& -& -\\ % pvtv2
AS-MLP-T \cite{lian2021asmlp} & 86 & 739
    &- &- &- &- &- &-
    & 50.1 & 68.8 & 54.3 & 43.5 & 66.3 & 46.9 \\ % asmlp
Shift-T \cite{wang2022shift} & 86 & 743
    &- &- &- &- &- &-
    & 50.3 & 68.6 & 54.7 & 43.4 & 66.2 & 47.0 \\
\oursxt & 73 & 693
    & 47.6 & 66.5 & 51.4 & 41.3 & 63.6 & 44.6
    & 50.0 & 68.7 & 54.4 & 43.5 & 66.2 & 46.8 \\
\ourst & 85 & 730
    & \textbf{49.4} & \textbf{68.3} & \textbf{53.4} & \textbf{42.8} & \textbf{65.7} & \textbf{45.9}
    & \textbf{51.3} & \textbf{70.4} & \textbf{55.6} & \textbf{44.6} & \textbf{67.7} & \textbf{48.4} \\ % done
\midrule

% X101-64 \cite{xie2017ResNeXt} & 140 & 972
%     &- &- &- &- &- &-
%     & 48.3 & 66.4 & 52.3 & 41.7 & 64.0 & 45.1 \\ % cswin
Swin-B \cite{liu2021swin} & 145 & 982 
    & 50.8 & 70.1 & 55.1 & 43.9 & 67.4 & 47.4
    & 51.9 & 70.5 & 56.4 & 45.0 & 68.1 & 48.9 \\
ConvNeXt-B \cite{liu2022convnext} & 146 & 964
    &- &- &- &- &- &-
    & 52.7 & 71.3 & 57.2 & 45.6 & 68.9 & 49.5 \\
ASMLP-B \cite{lian2021asmlp} & 145 & 961 
    &- &- &- &- &- &-
    & 51.5 & 69.8 & 55.8 & 44.6 & 67.6 & 48.2 \\
\ourss & 96 & 790
    & 51.0 & 70.3 & 55.4 & 44.2 & 67.5 & 47.6
    & 51.5 & 70.3 & 55.9 & 44.8 & 68.0 & 48.6 \\
\arrayrulecolor{white}\hline\arrayrulecolor{black}
\oursb & 110 & 856 
    & 51.3 & 70.4 & 55.7 & 44.6 & 68.0 & 48.2 
    & 52.5 & 71.6 & 57.0 & 45.6 & 69.1 & 49.5 \\
\arrayrulecolor{white}\hline\arrayrulecolor{black}
\oursl & 134 & 902 
    & \textbf{51.8} & \textbf{70.9} & \textbf{56.3} & \textbf{44.8} & \textbf{68.4} & \textbf{48.4}
    & \textbf{53.3} & \textbf{72.1} & \textbf{57.9} & \textbf{46.3} & \textbf{69.8} & \textbf{50.4} \\ 


\bottomrule 
\end{NiceTabular}
% }

==> tables/coco_cascade_retina.tex <==
\begingroup

\renewcommand\arraystretch{1.1}
\resizebox{\textwidth}{!}{    
\setlength{\tabcolsep}{3pt}
\begin{NiceTabular}{@{}l@{\hskip1pt}|@{}c@{}|ccc|ccc|@{}c@{}|ccc|ccc@{\hskip1pt}}[code-before=
\rectanglecolor{\rc}{4-1}{4-15}
\rectanglecolor{\rc}{7-1}{7-15}
\rectanglecolor{\rc}{10-1}{11-15}
\rectanglecolor{\rc}{14-1}{14-15}
]
\hline
\rule{0pt}{1.1em}
\multirow{2}{*}{Model} &  \multicolumn{7}{c}{\normalsize Cascade Mask R-CNN 1$\times$ MS} & \multicolumn{7}{c}{\normalsize RetinaNet 3$\times$ MS} \\
% \cline{2-8}
% \cline{9-15}
  & 
  \begingroup
%   \scriptsize
  \#P.(M)
  \endgroup
  & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$^m$ & AP$^m_{50}$ & AP$^m_{75}$ & 
  \begingroup
%   \scriptsize
  \#P.(M)
  \endgroup
  & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$_S$ & AP$_{M}$ & AP$_{L}$ \\
\hline

PVT-T \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 23
    & 39.4 & 59.8 & 42.0 & 25.5 & 42.0 & 52.1 \\
\oursxt & 73 
    & 47.6 & 66.5 & 51.4 & 41.3 & 63.6 & 44.6
    & 25
    & \textbf{43.7} & 64.7 & 46.7 & 28.9 & 47.4 & 57.4  \\
\hline

PVT-S \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 34
    & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2 \\
Swin-T \cite{liu2021swin} & 86 
    & 48.1 & 67.1 & 52.2 & 41.7 & 64.4 & 45.0 % github
    & 39
    & 45.0 & 65.9 & 48.4 & 29.7 & 48.9 & 58.1 \\ % focal
% TwinP-S \cite{chu2021twins} & -
%     & - & - & - & - & - & -
%     & 34
%     & 45.2 & 66.5 & 48.6 & 30.0 & 48.8 & 58.9 \\
% Twin-S \cite{chu2021twins} & -
%     & - & - & - & - & - & - 
%     & 34
%     & 45.6 & 67.1 & 48.6 & 29.8 & 49.3 & 60.0 \\
\ourst & 85
    & \textbf{49.4} & 68.3 & 53.4 & \textbf{42.8} & 65.7 & 45.9
    & 37
    & \textbf{45.8} & 66.9 & 49.2 & 29.9 & 49.3 & 59.9 \\
\hline

PVT-M \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 54
    & 43.2 & 63.8 & 46.1 & 27.3 & 46.3 & 58.9 \\
Swin-S \cite{liu2021swin} & 107 
    & 50.1 & 69.3 & 54.2 & 43.2 & 66.4 & 46.8 % ours
    & 60 
    & 46.4 & 67.0 & 50.1 & 31.0 & 50.1 & 60.3 \\ %focal
% TwinsP-B \cite{chu2021twins} & -
%     & - & - & - & - & - & - 
%     & 54
%     & 46.4 & 67.7 & 49.8 & 31.3 & 50.2 & 61.4 \\
% Twins-B \cite{chu2021twins} & -
%     & - & - & - & - & - & - 
%     & 67
%     & 46.9 & 68.0 & 50.2 & 31.7 & 50.3 & 61.8 \\
\ourss & 96 
    & 51.0 & 70.3 & 55.4 & 44.2 & 67.5 & 47.6
    & 47
    & 46.3 & 68.0 & 49.5 & 30.4 & 50.6 & 59.9 \\
\arrayrulecolor{white}\hline
\oursb & 110
    & \textbf{51.3} & 70.4 & 55.7 & \textbf{44.6} & 68.0 & 48.2
    & 62 
    & \textbf{46.6} & 67.7 & 50.1 & 30.4 & 50.4 & 61.0 \\
\arrayrulecolor{black}\hline

PVT-L \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 71
    & 43.4 & 63.6 & 46.1 & 26.1 & 46.0 & 59.5 \\
Swin-B \cite{liu2021swin} & 145 
    & 50.8 & 70.1 & 55.1 & 43.9 & 67.4 & 47.4
    & 98 
    & 45.8 & 66.4 & 49.1 & 29.9 & 49.4 & 60.3 \\ %focal
\oursl & 134 is 
    & \textbf{51.8} & 70.9 & 56.3 & \textbf{44.8} & 68.4 & 48.4
    & 86 
    & \textbf{47.5} & 68.8 & 51.2 & 31.5 & 51.4 & 62.0 \\
\hline

\end{NiceTabular}
}
\vspace{-0.3cm}
\endgroup

==> tables/coco_mask1xms.tex <==
\begingroup

% \begi
\resizebox{\textwidth}{!}{    
\begin{NiceTabular}{@{}l@{}|@{}c@{}|ccc|ccc|@{}c@{}|ccc|ccc@{}}
\CodeBefore
\rectanglecolor{\rc}{4-1}{4-}
\rectanglecolor{\rc}{7-1}{7-}
\rectanglecolor{\rc}{10-1}{11-}
\rectanglecolor{\rc}{14-1}{14-}
\Body
\hline
\multirow{2}{*}{Model} &  \multicolumn{7}{c}{Mask R-CNN 1$\times$ MS} & \multicolumn{7}{c}{RetinaNet 3$\times$} \\
\cline{2-8}
\cline{9-15}
  & 
  \begingroup
  \scriptsize
  \#P/M
  \endgroup
  & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$^m$ & AP$^m_{50}$ & AP$^m_{75}$ & 
  \begingroup
  \scriptsize
  \#P/M
  \endgroup
  & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$_S$ & AP$_{M}$ & AP$_{L}$ \\
\hline

PVT-T \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 23
    & 39.4 & 59.8 & 42.0 & 25.5 & 42.0 & 52.1 \\
\oursxt & 35
    & 42.9 & 65.5 & 47.0 & 39.3 & 62.3 & 42.1
    & 25
    & \textbf{43.7} & 64.7 & 46.7 & 28.9 & 47.4 & 57.4  \\
\hline

PVT-S \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 34
    & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2 \\
Swin-T \cite{liu2021swin} & 48
    & 43.7 & 66.6 & 47.7 & 39.8 & 63.3 & 42.7 % github
    & 39
    & 45.0 & 65.9 & 48.4 & 29.7 & 48.9 & 58.1 \\ % focal
% TwinP-S \cite{chu2021twins} & -
%     & - & - & - & - & - & -
%     & 34
%     & 45.2 & 66.5 & 48.6 & 30.0 & 48.8 & 58.9 \\
% Twin-S \cite{chu2021twins} & -
%     & - & - & - & - & - & - 
%     & 34
%     & 45.6 & 67.1 & 48.6 & 29.8 & 49.3 & 60.0 \\
\ourst & 47
    & \textbf{45.8} & 68.3 & 50.3 & \textbf{41.6} & 65.2 & 44.2
    & 37
    & \textbf{45.8} & 66.9 & 49.2 & 29.9 & 49.3 & 59.9 \\
\hline

PVT-M \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 54
    & 43.2 & 63.8 & 46.1 & 27.3 & 46.3 & 58.9 \\
Swin-S \cite{liu2021swin} & 69
    & 46.4 & 68.9 & 51.1 & 41.7 & 65.5 & 44.8 
    & 60 
    & 46.4 & 67.0 & 50.1 & 31.0 & 50.1 & 60.3 \\ %focal
% TwinsP-B \cite{chu2021twins} & -
%     & - & - & - & - & - & - 
%     & 54
%     & 46.4 & 67.7 & 49.8 & 31.3 & 50.2 & 61.4 \\
% Twins-B \cite{chu2021twins} & -
%     & - & - & - & - & - & - 
%     & 67
%     & 46.9 & 68.0 & 50.2 & 31.7 & 50.3 & 61.8 \\
\ourss & 58
    & 46.8 & 69.2 & 51.4 & 42.5 & 66.3 & 45.8
    & 47
    & 46.3 & 68.0 & 49.5 & 30.4 & 50.6 & 59.9 \\
\arrayrulecolor{white}\hline
\oursb & 72
    & \textbf{47.0} & 69.6 & 51.7 & \textbf{42.7} & 66.6 & 46.0
    & 62 
    & \textbf{46.6} & 67.7 & 50.1 & 30.4 & 50.4 & 61.0 \\
\arrayrulecolor{black}\hline

PVT-L \cite{wang2021pyramidpvt} & -
    & - & - & - & - & - & -
    & 71
    & 43.4 & 63.6 & 46.1 & 26.1 & 46.0 & 59.5 \\
Swin-B \cite{liu2021swin} & 107
    & 46.9 & 69.8 & 51.2 & 42.1 & 66.3 & 44.9
    & 98 
    & 45.8 & 66.4 & 49.1 & 29.9 & 49.4 & 60.3 \\ %focal
\oursl & 96
    & \textbf{47.7} & 70.3 & 52.4 & \textbf{43.1} & 67.5 & 46.2
    & 86 
    & \textbf{47.5} & 68.8 & 51.2 & 31.5 & 51.4 & 62.0 \\
\hline

\end{NiceTabular}
}
\vspace{-0.3cm}
\endgroup

==> tables/coco_mask_all.tex <==
% \setlength{\tabcolsep}{10pt}
% \resizebox{\textwidth}{!}{


\small
\begin{NiceTabular}{@{}lcccccccccccccc@{}}[code-before=
\rectanglecolor{\rc}{9-1}{10-15}
\rectanglecolor{\rc}{16-1}{18-15}
]
\toprule
\multirow{2}{*}{Backbone} & \Block{2-1}{\makecell{\#Params.\\(M)}} & \multirow{2}{*}{\makecell{FLOPs\\{(G)}}} & \multicolumn{6}{c}{\normalsize Mask R-CNN 1$\times$} & \multicolumn{6}{c}{\normalsize Mask R-CNN 3$\times$ MS} \\
& & & \textbf{AP$^b$} & AP$^b_{50}$ & AP$^b_{75}$ & \textbf{AP$^m$} & AP$^m_{50}$ & AP$^m_{75}$ & \textbf{AP$^b$} & AP$^b_{50}$ & AP$^b_{75}$ & \textbf{AP$^m$} & AP$^m_{50}$ & AP$^m_{75}$ \\

\arrayrulecolor{black}\midrule\arrayrulecolor{black}

% ResNet-50 \cite{he2016deepresnet} & 44 & 260 % wave 
%     & 38.0 & 58.6 & 41.4 & 34.4 & 55.1 & 36.7
%     & 41.0 & 61.7 & 44.9 & 37.1 & 58.4 & 40.1 \\  % cswin
% PVT-S & 44 & 245 % cswin 
%     & 40.4 & 62.9 & 43.8 & 37.8 & 60.1 & 40.3 
%     & 43.0 & 65.3 & 46.9 & 39.9 & 62.5 & 42.8 \\ % cswin
Swin-T \cite{liu2021swin} & 48 & 264 % cswin
    & 42.2 & 64.6 & 46.2 & 39.1 & 61.6 & 42.0 
    & 46.0 & 68.2 & 50.2 & 41.6 & 65.1 & 44.8 \\ % cswin
ConvNeXt-T \cite{liu2022convnext} & 48 & 262 
    &- &- &- &- &- &-
    & 46.2 & 67.9 & 50.8 & 41.7 & 65.0 & 44.9 \\
% TwinsP-S & 44 & 245 % cswin 
    % & 42.9 & 65.8 & 47.1 & 40.0 & 62.7 & 42.9 
    % & 46.8 & 69.3 & 51.8 & 42.6 & 66.3 & 46.0 \\ % cswin
Twins-S \cite{chu2021twins} & 44 & 228 % cswin
    & 43.4 & 66.0 & 47.3 & 40.3 & 63.2 & 43.4 
    & 46.8 & \textbf{69.2} & 51.2 & 42.6 & 66.3 & 45.8 \\ % cswin
% PVTv2-B2 \cite{wang2021pvtv2} & 45 & - 
    % & 45.3 & 67.1 & 49.6 & 41.2 & 64.2 & 44.4 
    % & & & & & & \\ % pvtv2
% ViL-S \cite{zhang2021ViL} & 45 % csin
%     & 44.9 & 67.1 & 49.3 & 41.0 & 64.2 & 44.1 
%     & 36 % github
%     & 44.2 & 65.2 & 47.6 & 28.8 & 48.0 & 57.8 \\ 
ASMLP-T \cite{lian2021asmlp} & 48 & 260
    &- &- &- &- &- &-
    & 46.0 & 67.5 & 50.7 & 41.5 & 64.6 & 44.5 \\ % asmlp
CycleMLP-B2 \cite{chen2022cyclemlp} & 47 & 250  % wave
    & 42.1 & 64.0 & 45.7 & 38.9 & 61.2 & 41.8 
    &- &- &- &- &- &- \\ % cycle
WaveMLP-S \cite{tang2021imagewavemlp} & 47 & 250
    & 44.0 & 65.8 & 48.2 & 40.0 & 63.1 & 42.9 
    &- &- &- &- &- &- \\ % wavemlp
% Shift-T \cite{wang2022shift} & 48 & -
%     & 45.4 & -    & -    & 40.9 & -    & - 
%     & 47.1 & - & - & 42.3 & - & - \\ % shift
\oursxt & 35 & 215
    & 42.8 & 64.9 & 46.9 & 39.5 & 62.1 & 42.5
    & 45.0 & 67.4 & 49.5 & 41.1 & 64.4 & 44.2 \\ 
\arrayrulecolor{white}\hline\arrayrulecolor{black}
\ourst & 47 & 251
    & \textbf{44.8} & \textbf{66.9} & \textbf{49.0} & \textbf{41.0} & \textbf{64.2} & \textbf{44.3}
    & \textbf{47.1} & 69.0 & \textbf{51.7} & \textbf{42.7} & \textbf{66.5} & \textbf{46.0} \\ % done
% \hline

\midrule

% X101-64 \cite{xie2017ResNeXt} & 102 & 493 
%     & 42.8 & 63.8 & 47.3 & 38.4 & 60.6 & 41.3
%     & 44.4 & 64.9 & 48.8 & 39.7 & 61.9 & 42.6  \\ % cswin
% PVT-L  & 81 & 364 % cswin
%     & 42.9 & 65.0 & 46.6 & 39.5 & 61.9 & 42.5 
%     & 44.5 & 66.0 & 48.3 & 40.7 & 63.4 & 43.7  \\
% ViL-B \cite{zhang2021ViL} & 76 % csin
%     & 45.1 & - & - & 41.0 & - & - 
%     & 
%     & 45.7 & 67.2 & 49.9 & 41.3 & 64.4 & 44.5 \\
% TwinsP-L & 81 & 364
%     & 45.4 & - & - & 41.5 & - & -
%     &-& -&- &- &- &- \\
Twins-L \cite{chu2021twins} & 120 & 474
    & 45.9 & - & - & 41.6 & - & -
    & - &- &- &- &- &-  \\
Swin-B \cite{liu2021swin} & 107 & 496
    & 45.5 & - & - & 41.3 & - & - % twins
    & 48.5 & 69.8 & 53.2 & 43.4 & 66.8 & 46.9  \\
% Focal-B & 110 & 533 & 47.8 & 70.2 & 52.5 & 43.2 & 67.3 & 46.5 
%         & 49.0 & 70.1 & 53.6 & 43.7 & 67.6 & 47.0 \\
MViT-B \cite{yan2022MViT} & 73 & 438 
    &- &- &- &- &- &-
    & 48.8 & 71.2 & 53.5 & 44.2 & 68.4 & 47.6 \\
% CycleMLP-B4 \cite{chen2022cyclemlp} & 72 % wave | flops: our
%     & 44.1 & 65.7 & 48.1 & 40.2 & 62.7 & 43.5
%     & 62
%     & 43.2 & 63.9 & 46.2 & 26.6 & 46.5 & 57.4 \\
CycleMLP-B5 \cite{chen2022cyclemlp} & 95 & 421 % wave
    & 44.1 & 65.5 & 48.4 & 40.1 & 62.8 & 43.0
    &- &- &- &- &- &-   \\
WaveMLP-B \cite{tang2021imagewavemlp} & 75 & 353
    & 45.7  & 67.5 & 50.1 & 27.8 & 49.2 & 59.7
    &- &- &- &- &- &-  \\

% \ourss & 58 & 311
%     & 46.0 & 68.2 & 50.4 & 42.0 & 65.3 & 45.5
%     & 48.1 & 69.7 & 52.9 & 43.4 & 67.2 & 46.7 \\
\arrayrulecolor{white}
\hline
\arrayrulecolor{black}
\ourss & 58 & 311
    & 46.0 & 68.2 & 50.4 & 42.0 & 65.3 & 45.5
    & 48.1 & 69.7 & 52.9 & 43.4 & 67.2 & 46.7 \\
\oursb & 72 & 377
    & 46.5 & 68.6 & 51.0 & 42.5 & 66.1 & 45.8 
    & 49.0 & 70.7 & 54.0 & 43.9 & 67.7 & 47.5 \\
\arrayrulecolor{white}\hline\arrayrulecolor{black}
\oursl & 96 & 424
    & \textbf{47.4} & \textbf{69.9} & \textbf{52.0} & \textbf{43.2} & \textbf{67.3} & \textbf{46.5}
    & \textbf{49.5} & \textbf{71.5} & \textbf{54.3} & \textbf{44.5} & \textbf{68.7} & \textbf{48.1} \\

\bottomrule
\end{NiceTabular}
% }





==> tables/coco_retina.tex <==
\begingroup

\resizebox{\textwidth}{!}{    
\begin{NiceTabular}{l|@{}cc@{}|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\makecell{Param\\(M)}} & \multirow{2}{*}{\makecell{FLOPs\\(G)}} & \multicolumn{6}{c|}{RetinaNet 1$\times$} & \multicolumn{6}{c}{RetinaNet 3$\times$ MS} \\
\cline{4-15}
 & & & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$  \\
\hline
ResNet-18 \cite{he2016deepresnet} & 22 & 189 
    & 31.8 & 49.6 & 33.6 & 16.3 & 34.3 & 43.2 
    & 35.4 & 53.9 & 37.6 & 19.5 & 38.2 & 46.8 \\ % wave | pvt
PVT-T \cite{wang2021pyramidpvt} & 23 & 190 
    & 36.7 & 56.9 & 38.9 & 22.6 & 38.8 & 50.0
    & 39.4 & 59.8 & 42.0 & 25.5 & 42.0 & 52.1 \\ % wave | pvt
CycleMLP-B1 \cite{chen2022cyclemlp} & 25 & 195 
    & 38.6 & 59.1 & 40.8 & 21.9 & 41.8 & 50.7 
    &- &- &- &- &- &-\\ % wave
WaveMP-T \cite{tang2021imagewavemlp} & 25 & 196 
    & 40.4 & 61.0 & 43.4 & 24.9 & 43.7 & 51.7 
    &- &- &- &- &- &-\\ % wave
\rowcolor{Gray!25}\oursxt & - & -
    & 41.2 & 62.3 & 43.7 & 24.4 & 45.3 & 54.2
    & 43.7 & 64.7 & 46.7 & 28.9 & 47.4 & 57.4 \\ % done
\hline

ResNet-50 \cite{he2016deepresnet} & 38 & 239
    & 36.3 & 55.3 & 38.6 & 19.3 & 40.0 & 48.8
    & 39.0 & 58.4 & 41.8 & 22.4 & 42.8 & 51.6 \\ % wave | pvt
Swin-T \cite{liu2021swin} & 29 & 245
    & 41.5 & 62,1 & 44.2 & 25.1 & 44.9 & 55.5
    &- &- &- &- &- &-\\ % wave
PVT-S \cite{wang2021pyramidpvt} & 34 & 227 
    & 40.4 & 61.3 & 43.0 & 25.0 & 42.9 & 55.7 
    & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2 \\ % wave
CycleMLP-B2 \cite{chen2022cyclemlp} & 37 & 231 
    & 40.9 & 61.8 & 43.4 & 23.4 & 44.7 & 53.4 
    &- &- &- &- &- &-\\ % wave
% WaveMLP-S \cite{tang2021imagewavemlp} & 37 & 231 
%     & 43.4 & 64.4 & 46.5 & 26.6 & 47.1 & 57.1
%     & & & & & & \\ % wave
\rowcolor{Gray!25}\ours & - & -
    & 43.6 & 64.9 & 46.8 & 27.2 & 47.5 & 57.9
    & 45.8 & 66.9 & 49.2 & 29.9 & 49.3 & 59.9 \\ % done
\hline


ResNet101 \cite{he2016deepresnet} & 56.7 & 149 % twins
    & 38.5 & 57.8 & 41.2 & 21.4 & 42.6 & 51.1
    & 40.9 & 60.1 & 44.0 & 23.7 & 45.0 & 53.8 \\
ResNeXt101-32x4d \cite{xie2017ResNeXt} & 56.4 & 151 % twins
    & 39.9 & 59.6 & 42.7 & 22.3 & 44.2 & 52.5
    & 41.4 & 61.0 & 44.3 & 23.9 & 45.5 & 53.7 \\
PVT-M \cite{wang2021pyramidpvt} & 53.9 & 151 % twins
    & 41.9 & 63.1 & 44.3 & 25.0 & 44.9 & 57.6
    & 43.2 & 63.8 & 46.1 & 27.3 & 46.3 & 58.9 \\
TwinsP-B \cite{chu2021twins} & 54.1 & 151 
    & 44.3 & 65.6 & 47.3 & 27.9 & 47.9 & 59.6
    & 46.4 & 67.7 & 49.8 & 31.3 & 50.2 & 61.4 \\
Twin-B \cite{chu2021twins} & 67.0 & 163 
    & 45.3 & 66.7 & 48.1 & 28.5 & 48.9 & 60.6
    & 46.9 & 68.0 & 50.2 & 31.7 & 50.3 & 61.8 \\
Swin-B \cite{liu2021swin} & 59.8 & 162 % twins
    & 44.5 & 65.7 & 47.5 & 27.4 & 48.0 & 59.9
    & 46.3 & 67.4 & 49.8 & 31.1 & 50.3 & 60.9 \\
CycleMLP-B3 \cite{chen2022cyclemlp} & 48.1 & - % wave 
    & 42.5 & 63.2 & 45.3 & 25.2 & 45.5 & 56.2
    &- &- &- &- &- &- \\
WaveMLP-M \cite{tang2021imagewavemlp} & 49.4 & - % wave
    & 44.8 & 65.8 & 47.8 & 28.0 & 48.2 & 59.1
    &- &- &- &- &- &- \\

\rowcolor{Gray!25}
\ourss & - & -     
    & 44.9 & 66.1 & 48.1 & 27.3 & 48.8 & 59.2 
    & 45.7 & 67.3 & 48.8 & 30.0 & 50.0 & 59.5 \\
\rowcolor{Gray!25}
\oursb & - & - 
    & 45.2 & 66.7 & 48.4 & 28.1 & 49.1 & 59.9
    & 46.6 & 67.7 & 50.1 & 30.4 & 50.4 & 61.0 \\
\rowcolor{Gray!25}
\oursl & & 
    & 45.5 & 67.2 & 48.8 & 29.9 & 49.5 & 59.7 
    & 47.5 & 68.8 & 51.2 & 31.5 & 51.4 & 62.0 \\

\bottomrule
\end{NiceTabular}
}

\endgroup

==> tables/coco_retina_all.tex <==
\begingroup
\small
% \resizebox{\textwidth}{!}{    
\begin{NiceTabular}{@{}lcccccccccccccc@{}}[code-before=
\rectanglecolor{\rc}{7-1}{8-15}
\rectanglecolor{\rc}{13-1}{15-15}
]
\toprule
\multirow{2}{*}{Backbone} & \Block{2-1}{\makecell{\#Params.\\(M)}} & \multirow{2}{*}{\makecell{FLOPs\\{(G)}}} & \multicolumn{6}{c}{\normalsize RetinaNet 1$\times$} & \multicolumn{6}{c}{\normalsize RetinaNet 3$\times$ MS} \\
& & 
& \textbf{AP$^b$} & AP$^b_{50}$ & AP$^b_{75}$ 
& AP$_S$ & AP$_{M}$ & AP$_{L}$
& \textbf{AP$^b$} & AP$^b_{50}$ & AP$^b_{75}$ 
& AP$_S$ & AP$_{M}$ & AP$_{L}$ \\
\midrule

% ResNet-50 \cite{he2016deepresnet} & 38 & 239
%     & 36.3 & 55.3 & 38.6 & 19.3 & 40.0 & 48.8 
%     & 39.0 & 58.4 & 41.8 & 22.4 & 42.8 & 51.6 \\% twins
% PVT-S  & 34 & 227 
%     & 40.4 & 61.3 & 43.0 & 25.0 & 42.9 & 55.7 
%     & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2 \\% ppvt
Swin-T \cite{liu2021swin} & 39 & 245 
    & 41.5 & 62,1 & 44.2 & 25.1 & 44.9 & 55.5
    & 45.0 & 65.9 & 48.4 & 29.7 & 48.9 & 58.1\\ % focal
Twins-S \cite{chu2021twins} & 34 & 286
    & 43.0 & 64.1 & 46.0 & \textbf{27.5} & 46.3 & 57.3 
    & 45.2 & 66.5 & 48.6 & 30.0 & 48.8 & 58.9 \\% twins
% Twins-S \cite{chu2021twins} & 34 & 236
%     & 43.0 & 64.2 & 46.3 & \textbf{28.0} & 46.4 & 57.5 
%     & 45.6 & \textbf{67.1} & 48.6 & 29.8 & \textbf{49.3} & \textbf{60.0} \\%twins
% PVTv2-B2 \cite{wang2021pvtv2} & 45 & - 
    % & 45.3 & 67.1 & 49.6 & 41.2 & 64.2 & 44.4 
    % & & & & & & \\ % pvtv2
CycleMLP-B2 \cite{chen2022cyclemlp} & 37 & 231
    & 40.9 & 61.8 & 43.4 & 23.4 & 44.7 & 53.4
    & - & - & - & - & - & - \\ % cycle
WaveMLP-S \cite{tang2021imagewavemlp} & 37 & 231
    & 43.4 & 64.4 & 46.5 & 26.6 & 47.1 & 57.1
    & - & - & - & - & - & -  \\ % wavemlp
\oursxt & 25 & 196
    & 41.2 & 62.3 & 43.7 & 24.4 & 45.3 & 54.2 
    & 43.7 & 64.7 & 46.7 & 28.9 & 47.4 & 57.4 \\ % done
\arrayrulecolor{white}\hline\arrayrulecolor{black}
\ourst & 37 & 233
    & \textbf{43.6} & \textbf{64.9} & \textbf{46.8} & 27.2 & \textbf{47.5} & \textbf{57.9}
    & \textbf{45.8} & \textbf{66.9} & \textbf{49.2} & \textbf{29.9} & \textbf{49.3} & \textbf{59.9 }\\ % done
\midrule

% X101-64 \cite{xie2017ResNeXt} & 96 &473
%     & 41.0 & 60.9 & 44.0 & 23.9 & 45.2 & 54.0
%     & 41.8 & 61.5 & 44.4 & 25.2 & 45.4 & 54.6\\%focal
% PVT-L  & 71 & 345
%     & 42.6 & 63.7 & 45.4 & 25.8 & 46.0 & 58.4
%     & 43.4 & 63.6 & 46.1 & 26.1 & 46.0 & 59.5 \\
% ViL-B \cite{zhang2021ViL} & 76 % csin
%     & 45.1 & - & - & 41.0 & - & - 
%     & 
%     & 45.7 & 67.2 & 49.9 & 41.3 & 64.4 & 44.5 \\
% TwinsP-L  & 71 & 476
%     & 45.1 & 66.4 & 48.4 & - & - & - 
%     & - &- &- &- &- &- \\
Twins-L \cite{chu2021twins} & 111 & 528
    & 45.7 & 67.1 & 49.2 & - & - & - 
    & - &- &- &- &- &- \\
Swin-B \cite{liu2021swin} & 98 & 477
    & 44.7 & 65.9 & 47.8 & - & - & - 
    & 45.8 & 66.4 & 49.1 & 29.9 & 49.4 & 60.3 \\
% CycleMLP-B4  & 72 % wave | flops: our
%     & 44.1 & 65.7 & 48.1 & 40.2 & 62.7 & 43.5
%     & 62
%     & 43.2 & 63.9 & 46.2 & 26.6 & 46.5 & 57.4 \\
CycleMLP-B5 \cite{chen2022cyclemlp}  & 86 & 402
    & 42.7 & 63.3 & 45.3 & 24.1 & 46.3 & 57.4  
    & - &- &- &- &- &- \\
WaveMLP-B \cite{tang2021imagewavemlp} & 66 & 334
    & 44.2 & 65.1 & 47.1 & 27.1 & 47.8 & 58.9 
    & - &- &- &- &- &- \\
\ourss & 48 & 293
    & 45.4 & 66.7 & 48.5 & 28.3 & 49.7 & 59.7 
    & {46.3} & 68.0 & 49.5 & 30.4 & 50.6 & 59.9 \\
\arrayrulecolor{white}\hline\arrayrulecolor{black}
\oursb & 62 & 359
    & 45.6 & 67.2 & 48.9 & 28.9 & 49.6 & 60.5 
    & {47.7} & 69.2 & 50.9 & \textbf{33.1} & 51.6 & 61.8 \\
\arrayrulecolor{white}\hline\arrayrulecolor{black}
\oursl & 86 & 405
    & \textbf{46.1} & \textbf{67.4} & \textbf{49.4} & \textbf{29.9} & \textbf{50.1} & \textbf{61.0} 
    & \textbf{48.1} & \textbf{69.5} & \textbf{51.8} & 31.7 & \textbf{52.1} & \textbf{63.0} \\

\bottomrule 
\end{NiceTabular}
% }
\endgroup

==> tables/fpn_back.tex <==
\begingroup

\begin{tabular}{@{}>{\columncolor{white}[0pt][\tabcolsep]}c@{}}

% \hfill{0.01\textwidth}
\hspace{0.06\textwidth}
\begin{minipage}{0.5\linewidth}
\begin{NiceTabular}{@{}lcccc@{}}[code-before=
\rectanglecolor{\rc}{7-1}{7-5}
\rectanglecolor{\rc}{18-1}{18-5}
]
\hline
Model & Arch. & \#P & FLOPs & mIoU  \\


\hline
ResNet18 
    & CNN   & 15.5 & 32 & 32.9 \\  % pvt
PVT-T 
    & Trans & 17.0 & 33 & 35.7 \\
P2T-T 
    & Trans & 14.9 & 32 & 39.5 \\
CycleMLP-B1 
    & MLP   & 18.9 & 33 & 40.8 \\
WaveMLP-T 
    & MLP   & 19.3 & - & 41.2 \\
\oursxt
    & MLP   & 19.1 & 33.1 & \textbf{43.0} \\
\hline


ResNet50  
    & CNN   & 28.5 & 46  & 36.7 \\  % pvt
PVT-S 
    & Trans & 28.2 & 45 & 39.8 \\
Swin-T   % twins
    & Trans & 31.9 & 46 & 41.5 \\
Twins-S 
    & Trans & 28.3 & 37 & 43.2 \\
TwinsP-S 
    & Trans & 28.4 & 40 & 44.3 \\
P2T-S 
    & Trans & 26.8 & 42 & 44.4 \\
GFNet-T 
    & FFT   & 26.6 & - & 41.0 \\
MorphMLP-T 
    & MLP   & 26.4 & - & 43.0 \\
CycleMLP-B2 
    & MLP & 30.6 & 42 & 43.4 \\ 
Wave-MLP-S   
    & MLP & 31.2 & - & 44.4 \\
\ourst
    & MLP   & 30.9 & 42.4 & \textbf{45.8} \\
\hline

% ResNet101 
%     & CNN & 47.5 & 65.1 & 38.8 \\
% % ResNeXt101-32$\times$4d 
% %     & CNN & 47.1 & 64.7 & 39.7 \\
% PVT-M \cite{wang2021pyramidpvt}
%     & Trans & 48.0 & 61.0 & 41.6 \\
% P2T-B 
%     & Trans & 39.9 & 57.5 & 46.2 \\
% Swin-S  
%     & Trans & 53.2 & 70 & 45.2 \\
% TwinsP-B 
%     & Trans & 48.1 & 55 & 44.9 \\
% Twins-B 
%     & Trans & 60.4 & 67 & 45.3 \\
% GFNet-S 
%     & FFT   & 47.5 & - & 42.5 \\ 
% CycleMLP-B3 
%     & MLP   & 42.1 & - & 44.3 \\
% CycleMLP-B4 
%     & MLP   & 55.6 & - & 45.1 \\
% WaveMLP-M 
%     & MLP   & 43.3 & - & 46.8 \\
% \rowcolor{\rc}
% \ourss 
%     & MLP   & - & - & 47.3 \\
% \hline


% % ResNeXt101-64$\times$4d 
% %     & CNN &  86.4 & 103.9 & 40.2 \\
% PVT-L 
%     & Trans & 65.1 & 79.6 & 42.1 \\
% TwinsP-L 
%     & Trans & 65.3 & 71 & 46.4 \\
% Swin-B 
%     & Trans & 91.2 & 107 & 46.0 \\ % twins
% Twins-L 
%     & Trans & 103.7 & 102 & 46.7 \\
% GFNet 
%     & FFT   & 74.7 & - & 44.8 \\
% CycleMLP-B5 
%     & MLP   & 79.4 & - & 45.5 \\
% \rowcolor{\rc}\oursb
%     & MLP   & - & - & 47.7 \\
% \arrayrulecolor{white}\hline
% \rowcolor{\rc}\oursl
%     & MLP   & - & - & 48.1 \\

% \arrayrulecolor{black}\hline
\end{NiceTabular}
		% }
\end{minipage}

%  ============================================== right
\begin{minipage}{0.5\linewidth}
% \resizebox{\textwidth}{!}{    
\begin{NiceTabular}{@{}lcccc@{}}[code-before=
\rectanglecolor{\rc}{9-1}{9-5}
\rectanglecolor{\rc}{17-1}{18-5}
]
\hline
Model & Arch. & \#P & FLOPs & mIoU  \\
% =============== FLOPs: 512x512


\hline
% ResNet18 
%     & CNN   & 15.5 & 32.2 & 32.9 \\  % pvt
% PVT-T 
%     & Trans & 17.0 & 33.2 & 35.7 \\
% P2T-T 
%     & Trans & 14.9 & 31.8 & 39.5 \\
% CycleMLP-B1 
%     & MLP   & 18.9 & - & 40.8 \\
% WaveMLP-T 
%     & MLP   & 19.3 & - & 41.2 \\
% \rowcolor{Gray!25}\oursxt
%     & MLP   & - & - & 43.0 \\
% \hline


% ResNet50  
%     & CNN   & 28.5 & 45.6  & 36.7 \\  % pvt
% Swin-T   % twins
%     & Trans & 31.9 & 46 & 41.5 \\
% PVT-S 
%     & Trans & 28.2 & 44.5 & 39.8 \\
% P2T-S 
%     & Trans & 26.8 & 41.7 & 44.4 \\
% Twins-S 
%     & Trans & 28.3 & 37 & 43.2 \\
% TwinsP-S 
%     & Trans & 28.4 & 40 & 44.3 \\
% GFNet-T 
%     & FFT   & 26.6 & - & 41.0 \\
% CycleMLP-T 
%     & MLP & 30.6 & - & 43.4 \\ 
% Wave-MLP-S   
%     & MLP & 31.2 & - & 44.4 \\
% \rowcolor{\rc}\ourst
%     & MLP   & & & 45.8 \\
% \hline

ResNet101 
    & CNN & 47.5 & 65 & 38.8 \\
% ResNeXt101-32$\times$4d 
%     & CNN & 47.1 & 64.7 & 39.7 \\
PVT-M 
    & Trans & 48.0 & 61 & 41.6 \\
TwinsP-B 
    & Trans & 48.1 & 55 & 44.9 \\
% P2T-B 
%     & Trans & 39.9 & 57.5 & 46.2 \\
Swin-S  
    & Trans & 53.2 & 70 & 45.2 \\
Twins-B 
    & Trans & 60.4 & 67 & 45.3 \\
% GFNet-S 
%     & FFT   & 47.5 & - & 42.5 \\ 
CycleMLP-B3 
    & MLP   & 42.1 & 58 & 44.3 \\
% CycleMLP-B4 
%     & MLP   & 55.6 & - & 45.1 \\
WaveMLP-M 
    & MLP   & 43.3 & - & 46.8 \\

\ourss 
    & MLP   & 42.4 & 57.8 & \textbf{47.3} \\
\hline


ResNeXt101 
    & CNN &  86.4 & 104 & 40.2 \\
PVT-L 
    & Trans & 65.1 & 80 & 42.1 \\
Swin-B 
    & Trans & 91.2 & 107 & 46.0 \\ % twins
TwinsP-L 
    & Trans & 65.3 & 71 & 46.4 \\
Twins-L 
    & Trans & 103.7 & 102 & 46.7 \\
% GFNet 
%     & FFT   & 74.7 & - & 44.8 \\
CycleMLP-B5 
    & MLP   & 79.4 & 86 & 45.5 \\
MorphMLP-B 
    & MLP   & 59.3 & - & 45.9 \\
\oursb
    & MLP   & 55.9 & 74.7 & \textbf{47.7} \\
\arrayrulecolor{white}\hline
\oursl
    & MLP   & 79.8 & 86.6 &\textbf{48.1} \\

\arrayrulecolor{black}\hline
\end{NiceTabular}
% }
\end{minipage}

\end{tabular}
\endgroup

==> tables/int_back.tex <==

\begin{tabular}{@{}c@{}}

\begin{minipage}[b]{0.5\textwidth}
\resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}l@{}|c|cc|c@{}}[code-before=
\rectanglecolor{\rc}{6-1}{6-5}
\rectanglecolor{\rc}{23-1}{23-5}
\rectanglecolor{\rc}{29-1}{29-5}
]
\hline
Model & Arch. & \makecell{\#P.\\(M)} & \makecell{FLOPs\\(G)} & \makecell{Top-1\\(\%)} \\
\hline
% ===================> xs
ResNet18\cite{he2016deepresnet}
		   	& CNN     & 12    & 1.8   & 69.8 \\
% EffNet-B3   & CNN   & 300$^2$   & 12    & 1.8   & 81.6 \\
PVTv2-B1 \cite{wang2021pvtv2}
            & Trans  & 13    & 2.1   & 78.7 \\
ResMLP-S12 \cite{touvron2021resmlp}
            & MLP    & 15    & 3.0   & 76.6 \\
CycleMLP-B1 \cite{chen2022cyclemlp} & MLP     & 15    & 2.1   & 78.9 \\
% \rowcolor{\rc}
\oursxt     & MLP      & 15    & 2.2   & \textbf{79.7} \\
\hline
% ===================> tiny
ResNet50\cite{he2016deepresnet}   
			& CNN     & 26    & 4.1   & 78.5 \\
Deit-S\cite{touvron2021deit}     
			& Trans   & 22    & 4.6   & 79.8 \\
PVT-S\cite{wang2021pyramidpvt}       
			& Trans   & 25    & 3.8   & 79.8 \\
Swin-T\cite{liu2021swin}
            & Trans   & 29    & 4.6   & 81.2 \\
TwinsP-S \cite{chu2021twins} & Trans & 24 
            & 3.8 & 81.2 \\
TNT-S \cite{han2021TNT}     & Trans   & 24    & 5.2   & 81.3 \\
Twins-S \cite{chu2021twins} 
            & Trans   & 24    & 2.9   & 81.7 \\
GFNet-H-S \cite{rao2021GFNet}
            & FFT     & 32    & 4.5   & 81.5 \\
% CvT-13      & Hybri   & 20    & 4.5   & 81.6 \\
EAMLP-14 \cite{guo2021EAMLP}
            & MLP    & 30    & - & 78.9 \\
ResMLP-S24 \cite{touvron2021resmlp}
            & MLP    & 30    & 6.0   & 79.4 \\
gMLP-S \cite{liu2021gMLP}
            & MLP    & 20    & 4.5   & 79.4 \\
ASMLP-T \cite{lian2021asmlp}
            & MLP    & 28    & 4.4   & 81.3 \\
ViP-S \cite{hou2021visionvip} % flops: morph
            & MLP     & 25    & 6.9     & 81.5 \\
MorphMLP-T \cite{zhang2021morphmlp}
            & MLP    & 23    & 3.9   & 81.6 \\
CycleMLP-B2\cite{chen2022cyclemlp} 
			& MLP     & 27    & 3.9   & 81.6 \\
Shift-T \cite{wang2022shift}
            & MLP     & 29    & 4.5   & 81.7 \\
% sMLP-T \cite{tang2021sparsesMLP}
%             & MLP  & 24    & 5.0   & 81.9 \\
% \rowcolor{\rc}
\ourst      & MLP     & 27    & 4.0   & \textbf{82.0} \\
\hline

PVT-M \cite{wang2021pyramidpvt}
            & Trans  & 44    & 6.7   & 81.2 \\
TwinsP-B \cite{chu2021twins}
            & Trans  & 44    & 6.7   & 82.7 \\
GFNet-B \cite{rao2021GFNet}
            & FFT    & 43    & 7.9   & 80.7 \\
MorphMLP-S \cite{zhang2021morphmlp}
            & MLP    & 38    & 7.0   & 82.6 \\
CycleMLP-B3 \cite{chen2022cyclemlp}
            & MLP    & 38    & 6.9   & 82.6 \\
% \rowcolor{\rc}
\ourss
            & MLP    & 39    & 6.9   & \textbf{83.0} \\
\hline


\end{NiceTabular}
}
\end{minipage}

% \vspace{0.02\linewidth}

\begin{minipage}[b]{0.5\textwidth}
\resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}l@{}|c|cc|c@{}}[code-before=
\rectanglecolor{\rc}{6-1}{6-5}
\rectanglecolor{\rc}{23-1}{23-5}
\rectanglecolor{\rc}{29-1}{29-5}
]
\hline
Model & Arch. & \makecell{\#P.\\(M)} & \makecell{FLOPs\\(G)} & \makecell{Top-1\\(\%)} \\
\hline

% ==================> small
PVT-L \cite{wang2021pyramidpvt}      & Trans   & 61    & 9.8   & 81.7 \\
Swin-S  \cite{liu2021swin}    & Trans   & 50    & 8.7   & 83.2 \\
Twins-B \cite{chu2021twins}
            & Trans  & 56    & 8.6   & 83.2 \\
GFNet-H-B \cite{rao2021GFNet}
            & FFT    & 54    & 8.4   & 82.9 \\
Mixer-B/16 \cite{tolstikhin2021mlpmixer}
            & MLP    & 59    & 12.7 & 76.4 \\
EAMLP-19 \cite{guo2021EAMLP}
            & MLP   & 55 & - & 79.4 \\
S$^2$MLP-D \cite{yu2022s2MLP}
            & MLP    & 51    & 10.5  & 80.7 \\
ViP-M \cite{hou2021visionvip} % flops: morph
            & MLP   & 55    & 16.3     & 82.7 \\
Shift-S \cite{wang2022shift}
            & MLP   & 50    & 8.8   & 82.8 \\
CycleMLP-B4 \cite{chen2022cyclemlp}
            & MLP   & 52    & 10.1  & 83.0 \\  
ASMLP-S \cite{lian2021asmlp}
            & MLP    & 50    & 8.5   & 83.1 \\
MorphMLP-B \cite{zhang2021morphmlp}
            & MLP    & 58    & 10.2  & 83.2 \\
% ConvNeXt-S \cite{liu2022convnext}
%             & Conv   & 50    & 8.7   & 83.1 \\
% sMLP-T \cite{tang2021sparsesMLP}
%             & MLP & 49    & 10.3  & 83.1 \\
% \rowcolor{\rc}
\oursb      & MLP     & 52    & 10.1  & \textbf{83.5} \\
\hline





% ==================> base
ViT-B/16$\dagger$ \cite{alexander2021vit}    & Trans   & 86    & 55.4  & 77.9 \\
Deit-B \cite{touvron2021deit}    & Trans   & 86    & 17.5  & 81.8 \\
CPVT-B \cite{chu2021CPVT} & Trans 
        & 88 & 17.6 & 82.3 \\
Deit-B$\dagger$ \cite{touvron2021deit}    & Trans  & 86    & 55.4  & 83.1 \\
Swin-B \cite{liu2021swin}    & Trans   & 88    & 15.4  & 83.5 \\
S$^2$MLP-W  \cite{yu2022s2MLP}
            & MLP    & 71    & 14.0  & 80.0 \\
ResMLP-B24 \cite{touvron2021resmlp}
            & MLP    & 116   & 23.0  & 81.0 \\
gMLP-B \cite{liu2021gMLP}
            & MLP    & 73    & 15.8  & 81.6 \\
CycleMLP-B5 \cite{chen2022cyclemlp} 
            & MLP & 76 & 15.3 & 83.1 \\
ViP-L \cite{hou2021visionvip}
            & MLP    & 88    & 24.4  & 83.2 \\
Shift-B \cite{wang2022shift}
            & MLP    & 89    & 15.6  & 83.3 \\
ASMLP-B \cite{lian2021asmlp}
            & MLP    & 88    & 15.2  & 83.3 \\

MorphMLP-L  & MLP    & 76    & 12.5  & 83.4 \\
CyceleMLP-B  \cite{chen2022cyclemlp}
            & MLP    & 88    & 15.2  & 83.4 \\ 
% sMLP-B \cite{tang2021sparsesMLP}
%             & MLP   & 66    & 14.0  & 83.4 \\
% \rowcolor{\rc}
\oursl      & MLP     & 76    & 12.3  & \textbf{83.6} \\
\hline

\end{NiceTabular}
}
\end{minipage}


\end{tabular}

\vspace{-0.5cm}

==> tables/int_sota.tex <==

\begin{tabular}{@{}c@{}}
\begin{minipage}[b]{0.48\textwidth}
\resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}lcccc@{}}[code-before=
\rectanglecolor{\rc}{5-1}{5-5}
\rectanglecolor{\rc}{20-1}{20-5}
\rectanglecolor{\rc}{26-1}{26-5}
]
\toprule
Model & Size & \makecell{\#P.(M)} & \makecell{FLOPs(G)} & \makecell{Top-1(\%)} \\



\midrule
ResNet18 \cite{he2016deepresnet}   
    & 224$^2$   & 12    & 1.8   & 69.8 \\
% EffNet-B3   & 224$^2$   & 300$^2$   & 12    & 1.8   & 81.6 \\
% PVTv2-B1    & 224$^2$   & 13    & 2.1   & 78.7 \\
ResMLP-S12 \cite{touvron2021resmlp}  
    & 224$^2$   & 15    & 3.0   & 76.6 \\
CycleMLP-B1 \cite{chen2022cyclemlp} 
    & 224$^2$   & 15    & 2.1   & 78.9 \\
\oursxt     & 224$^2$   & 15    & 2.2   & \textbf{79.7} \\



\midrule
ResNet50 \cite{he2016deepresnet, wightman2021resnettimm}    
    & 224$^2$   & 26    & 4.1   & 79.8 \\
Deit-S \cite{touvron2021deit}
    & 224$^2$   & 22    & 4.6   & 79.8 \\
Deit III-S \cite{touvron2022deit3}
    & 224$^2$   & 22    & 4.6   & 81.4 \\
PVT-S \cite{wang2021pyramidpvt}
    & 224$^2$   & 25    & 3.8   & 79.8 \\
Swin-T \cite{liu2021swin} 
    & 224$^2$   & 29    & 4.6   & 81.2 \\
TwinsP-S \cite{chu2021twins}
    & 224$^2$   & 24    & 3.8   & 81.2 \\
% TNT-S       & 224$^2$   & 24    & 5.2   & 81.3 \\
Twins-S \cite{chu2021twins} 
    & 224$^2$   & 24    & 2.9   & 81.7 \\
% GFNet-H-S   & 224$^2$   & 32    & 4.5   & 81.5 \\
% CvT-13      & Hybri   & 20    & 4.5   & 81.6 \\
% EAMLP-14    & 224$^2$   & 30    & -     & 78.9 \\
ResMLP-S24 \cite{touvron2021resmlp}
    & 224$^2$   & 30    & 6.0   & 79.4 \\
% gMLP-S      & 224$^2$   & 20    & 4.5   & 79.4 \\
ASMLP-T \cite{lian2021asmlp}
    & 224$^2$   & 28    & 4.4   & 81.3 \\
ViP-S \cite{hou2021visionvip}
    & 224$^2$   & 25    & 6.9   & 81.5 \\ % flops: morph
MorphMLP-T \cite{zhang2021morphmlp}
    & 224$^2$   & 23    & 3.9   & 81.6 \\
CycleMLP-B2 \cite{chen2022cyclemlp}
    & 224$^2$   & 27    & 3.9   & 81.6 \\
Shift-T \cite{wang2022shift}
    & 224$^2$   & 29    & 4.5   & 81.7 \\
sMLP-T \cite{tang2021sparsesMLP}
    & 224$^2$  & 24    & 5.0   & 81.9 \\
\ourst      & 224$^2$   & 27    & 4.0   & \textbf{82.0} \\



\midrule   
PVT-M \cite{wang2021pyramidpvt}
    & 224$^2$  & 44    & 6.7   & 81.2 \\
TwinsP-B \cite{chu2021twins}
    & 224$^2$  & 44    & 6.7   & 82.7 \\
% GFNet-B     &  224$^2$ & 43    & 7.9   & 80.7 \\
MorphMLP-S \cite{zhang2021morphmlp}
    & 224$^2$  & 38    & 7.0   & 82.6 \\
CycleMLP-B3 \cite{chen2022cyclemlp}
    & 224$^2$  & 38    & 6.9   & 82.6 \\
Deit III-M \cite{touvron2022deit3}
    & 224$^2$  & 39    & 8.0 & 83.0 \\    
\ourss      & 224$^2$  & 39    & 6.9   & \textbf{83.1} \\
\bottomrule
\end{NiceTabular}
}
\end{minipage}

\hspace{0.02\textwidth}

\begin{minipage}[b]{0.48\textwidth}
\resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}lcccc@{}}[code-before=
\rectanglecolor{\rc}{11-1}{11-5}
\rectanglecolor{\rc}{22-1}{22-5}
\rectanglecolor{\rc}{26-1}{26-5}
]
\toprule
Model & Size & \makecell{\#P.(M)} & \makecell{FLOPs(G)} & \makecell{Top-1(\%)} \\


\midrule
PVT-L \cite{wang2021pyramidpvt} 
    & 224$^2$   & 61    & 9.8   & 81.7 \\
Swin-S \cite{liu2021swin}
    & 224$^2$   & 50    & 8.7   & 83.2 \\
Twins-B \cite{chu2021twins}
    & 224$^2$   & 56    & 8.6   & 83.2 \\
% GFNet-H-B   & 224$^2$   & 54    & 8.4   & 82.9 \\
Mixer-B/16 \cite{tolstikhin2021mlpmixer} 
    & 224$^2$   & 59    & 12.7  & 76.4 \\
% EAMLP-19    & 224$^2$   & 55    & -     & 79.4 \\
% S$^2$MLP-D  & 224$^2$   & 51    & 10.5  & 80.7 \\
ViP-M \cite{hou2021visionvip}
    & 224$^2$   & 55    & 16.3  & 82.7 \\
Shift-S \cite{wang2022shift}
    & 224$^2$   & 50    & 8.8   & 82.8 \\
CycleMLP-B4 \cite{chen2022cyclemlp}
    & 224$^2$   & 52    & 10.1  & 83.0 \\[1pt]
ASMLP-S \cite{lian2021asmlp}
    & 224$^2$   & 50    & 8.5   & 83.1 \\[1pt]
MorphMLP-B \cite{zhang2021morphmlp}
    & 224$^2$   & 58    & 10.2  & 83.2 \\
% ConvNeXt-S & Conv      & 50    & 8.7   & 83.1 \\
% sMLP-T     & 224$^2$   & 49    & 10.3  & 83.1 \\
\oursb      & 224$^2$   & 52    & 10.1  & \textbf{83.5} \\



\midrule
Deit-B \cite{touvron2021deit}
    & 224$^2$   & 86    & 17.5  & 81.8 \\
Deit III-B \cite{touvron2022deit3}
    & 224$^2$   & 87    & 17.5  & \textbf{83.8} \\
% CPVT-B      & 224$^2$   & 88    & 17.6  & 82.3 \\
% Deit-B$\dagger$ 
            % & 224$^2$   & 86    & 55.4  & 83.1 \\
Swin-B \cite{liu2021swin}
    & 224$^2$   & 88    & 15.4  & 83.5 \\[1pt]
S$^2$MLP-W \cite{yu2022s2MLP}
    & 224$^2$   & 71    & 14.0  & 80.0 \\
% ResMLP-B24  & 224$^2$   & 116   & 23.0  & 81.0 \\
% gMLP-B      & 224$^2$   & 73    & 15.8  & 81.6 \\
CycleMLP-B5 \cite{chen2022cyclemlp}
    & 224$^2$   & 76    & 15.3  & 83.1 \\
ViP-L \cite{hou2021visionvip}
    & 224$^2$   & 88    & 24.4  & 83.2 \\
Shift-B \cite{wang2022shift}
    & 224$^2$   & 89    & 15.6  & 83.3 \\[1pt]
ASMLP-B \cite{lian2021asmlp}
    & 224$^2$   & 88    & 15.2  & 83.3 \\
MorphMLP-L \cite{zhang2021morphmlp}
    & 224$^2$   & 76    & 12.5  & 83.4 \\
% CyceleMLP-B & 224$^2$   & 88    & 15.2  & 83.4 \\ 
sMLP-B \cite{tang2021sparsesMLP} 
    & 224$^2$   & 66    & 14.0  & 83.4 \\
\oursl      & 224$^2$   & 76    & 12.3  & \textbf{83.8} \\
\hline
ViT-B/16$\uparrow$ \cite{alexander2021vit}
            & 384$^2$   & 86    & 55.4  & 77.9 \\
Deit-B$\uparrow$ \cite{touvron2021deit}
            & 384$^2$   & 86    & 55.4  & 83.1 \\
Swin-B$\uparrow$ \cite{liu2021swin}
            & 384$^2$   & 88    & 47.1  & 84.5 \\
\oursl$\uparrow$ 
            & 384$^2$   & 76    & 36.4  & \textbf{84.8} \\


\bottomrule
\end{NiceTabular}
}
\end{minipage}


\end{tabular}


==> tables/int_sota_two_size.tex <==

\begin{tabular}{@{}c@{}}

\begin{minipage}[b]{0.5\textwidth}
\resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}l@{}|c|ccc|c@{}}
\CodeBefore
\rectanglecolor{\rc}{6-1}{6-}
\rectanglecolor{\rc}{23-1}{23-}
\rectanglecolor{\rc}{28-1}{28-}
\Body
\hline
Model & Arch. & Scale & \makecell{\#P.\\(M)} & \makecell{FLOPs\\(G)} & Top-1 \\
\hline
% ===================> xs
ResNet18\cite{he2016deepresnet}
		   	& CNN   & \intsize   & 12    & 1.8   & 69.8 \\
% EffNet-B3   & CNN   & 300$^2$   & 12    & 1.8   & 81.6 \\
CycleMLP-B1 & MLP   & \intsize   & 15    & 2.1   & 78.9 \\
ResMLP-S12 \cite{touvron2021resmlp}
            & MLP   & \intsize  & 15    & 3.0   & 76.6 \\
PVTv2-B1 \cite{wang2021pvtv2}
            & Trans & -         & 13    & 2.1   & 78.7 \\
% \rowcolor{\rc}
\oursxt     & MLP    & \intsize   & 15    & 2.2   & \textbf{79.7} \\
\hline
% ===================> tiny
ResNet-50\cite{he2016deepresnet}   
			& CNN   & \intsize   & 26    & 4.1   & 78.5 \\
Deit-S\cite{touvron2021deit}     
			& Trans & \intsize   & 22    & 4.6   & 79.8 \\
Swin-T\cite{liu2021swin}
            & Trans & \intsize   & 29    & 4.6   & 81.2 \\
PVT-S\cite{wang2021pyramidpvt}       
			& Trans & \intsize   & 25    & 3.8   & 79.8 \\
TNT-S       & Trans & \intsize   & 24    & 5.2   & 81.3 \\
ResMLP-S24 \cite{touvron2021resmlp}
            & MLP   & \intsize  & 30    & 6.0   & 79.4 \\
CycleMLP-B2\cite{chen2022cyclemlp} 
			& MLP   & \intsize   & 27    & 3.9   & 81.6 \\
Twins-S \cite{chu2021twins} 
            & Trans & \intsize   & 24    & 2.8   & 81.7 \\
GFNet-H-S \cite{rao2021GFNet}
            & FFT   & \intsize   & 32    & 4.5   & 81.5 \\
Shift-T \cite{wang2022shift}
            & MLP   & -         & 29    & 4.5   & 81.7 \\
CvT-13      & Hybrid& \intsize  & 20    & 4.5   & 81.6 \\
EAMLP-14 \cite{guo2021EAMLP}
            & MLP   & \intsize  & 30    & - & 78.9 \\
ViP-S \cite{hou2021visionvip} % flops: morph
            & MLP   &           & 25    & 6.9     & 81.5 \\
% sMLP-T \cite{tang2021sparsesMLP}
%             & MLP   & -         & 24    & 5.0   & 81.9 \\
AS-MLP-T \cite{lian2021asmlp}
            & MLP   & \intsize  & 28    & 4.4   & 81.3 \\
MorphMLP-T \cite{zhang2021morphmlp}
            & MLP   & \intsize  & 23    & 3.9   & 81.6 \\
gMLP-S \cite{liu2021gMLP}
            & MLP   & \intsize  & 20    & 4.5   & 79.4 \\
% \rowcolor{\rc}
\ourst      & MLP   & \intsize   & 27    & 4.0   & 82.0 \\
\hline

PVT-M \cite{wang2021pyramidpvt}
            & Trans & \intsize  & 44    & 6.7   & 81.2 \\
GFNet-B \cite{rao2021GFNet}
            & FFT   & \intsize  & 43    & 7.9   & 80.7 \\
MorphMLP-S \cite{zhang2021morphmlp}
            & MLP   & \intsize  & 38    & 7.0   & 82.6 \\
CycleMLP-B3 \cite{chen2022cyclemlp}
            & MLP   & \intsize  & 38    & 6.9   & 82.6 \\
% \rowcolor{\rc}
\ourss
            & MLP   & \intsize  & 39    & 6.9   & 83.0 \\
\hline


\end{NiceTabular}
}
\end{minipage}

% \vspace{0.02\linewidth}

\begin{minipage}[b]{0.49\textwidth}
\resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}l@{}|c|ccc|c@{}}
\CodeBefore
\rectanglecolor{\rc}{15-1}{15-}
\rectanglecolor{\rc}{28-1}{28-}
\Body
\hline
Model & Arch. & Scale & \makecell{\#P.\\(M)} & \makecell{FLOPs\\(G)} & Top-1 \\
\hline

% ==================> small
Swin-S      & Trans & \intsize   & 50    & 8.7   & 83.0 \\
PVT-L       & Trans & \intsize   & 61    & 9.8   & 81.7 \\
Twins-B \cite{chu2021twins}
            & Trans & -         & 56    & 8.3   & 83.2 \\
Twins-B \cite{chu2021twins}
            & Trans &           & 56    & 8.6   & 83.2 \\
            
Shift-S \cite{wang2022shift}
            & MLP   & -         & 50    & 8.8   & 82.8 \\
CycleMLP-B4 \cite{chen2022cyclemlp}
            & MLP   & -         & 52    & 10.1  & 83.0 \\  
ViP-M \cite{hou2021visionvip} % flops: morph
            & MLP   &           & 55    & 16.3     & 82.7 \\
Mixer-B/16 \cite{tolstikhin2021mlpmixer}
            & MLP   & \intsize  & 59    & 12.7 & 76.4 \\
EAMLP-19 \cite{guo2021EAMLP}
            & MLP   & \intsize & 55 & - & 79.4 \\
AS-MLP-S \cite{lian2021asmlp}
            & MLP   & \intsize  & 50    & 8.5   & 83.1 \\
MorphMLP-B \cite{zhang2021morphmlp}
            & MLP   & \intsize  & 58    & 10.2  & 83.2 \\
S$^2$MLP-D \cite{yu2022s2MLP}
            & MLP   & \intsize  & 51    & 10.5  & 80.7 \\
GFNet-H-B \cite{rao2021GFNet}
            & FFT   & \intsize  & 54    & 8.4   & 82.9 \\
% ConvNeXt-S \cite{liu2022convnext}
%             & Conv  &           & 50    & 8.7   & 83.1 \\
% sMLP-T \cite{tang2021sparsesMLP}
%             & MLP   &           & 49    & 10.3  & 83.1 \\
% \rowcolor{\rc}
\oursb      & MLP   & \intsize   & 52    & 10.1  & 83.4 \\
\hline
% ==================> base
ViT-B/16    & Trans & 384$^2$   & 86    & 55.4  & 77.9 \\
Deit-B      & Trans & \intsize   & 86    & 17.5  & 81.8 \\
Deit-B      & Trans & $384^2$   & 86    & 55.4  & 83.1 \\
Swin-B      & Trans & \intsize   & 88    & 15.4  & 83.3 \\
Shift-B \cite{wang2022shift}
            & MLP   &-          & 89    & 15.6  & 83.3 \\
CyceleMLP-B  \cite{chen2022cyclemlp}
            & MLP   & -         & 88    & 15.2  & 83.2 \\  
ViP-L \cite{hou2021visionvip}
            & MLP   &           & 88    & 24.4  & 83.2 \\
ResMLP-B24 \cite{touvron2021resmlp}
            & MLP   & \intsize  & 116   & 23.0  & 81.0 \\
AS-MLP-B \cite{lian2021asmlp}
            & MLP   & \intsize  & 88    & 15.2  & 83.3 \\
gMLP-B \cite{liu2021gMLP}
            & mlp   & \intsize  & 73    & 15.8  & 81.6 \\
MorphMLP-L  & MLP   & \intsize  & 76    & 12.5  & 83.4 \\
S$^2$MLP-W  \cite{yu2022s2MLP}
            & MLP   & \intsize  & 71    & 14.0  & 80.0 \\
% sMLP-B \cite{tang2021sparsesMLP}
%             & MLP   &           & 66    & 14.0  & 83.4 \\
% \rowcolor{\rc}
\oursl      & MLP   & \intsize   & 76    & 12.3  & 83.6 \\
\hline

\end{NiceTabular}
}
\end{minipage}


\end{tabular}



==> tables/mask_back.tex <==

\begingroup

% \begin{subtable}[t]{\linewidth}
% \begi
\resizebox{\textwidth}{!}{    
\begin{NiceTabular}{@{}l@{}|@{}c@{}|ccc|ccc|@{}c@{}|ccc|ccc@{}}[code-before=
\rectanglecolor{\rc}{11-1}{11-5}
\rectanglecolor{\rc}{19-1}{19-5}
]
\hline
\multirow{2}{*}{Model} &  \multicolumn{7}{c}{Mask R-CNN 1$\times$} & \multicolumn{7}{c}{RetinaNet 1$\times$} \\
\cline{2-8}
\cline{9-15}
  & 
  \begingroup
  \scriptsize
  \#P/M
  \endgroup
  & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$^m$ & AP$^m_{50}$ & AP$^m_{75}$ & 
  \begingroup
  \scriptsize
  \#P/M
  \endgroup
  & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$_S$ & AP$_{M}$ & AP$_{L}$ \\
\hline

ResNet18 \cite{he2016deepresnet} & 31  % fp: our
    & 34.0 & 54.0 & 36.7 & 31.2 & 51.0 & 32.7
    & 21
    & 31.8 & 49.6 & 33.6 & 16.3 & 34.3 & 43.2  \\ % wavemlp | pvt
PVT-T \cite{wang2021pyramidpvt} & 33 
    & 36.7 & 59.2 & 39.3 & 35.1 & 56.7 & 37.3 
    & 23
    & 36.7 & 56.9 & 38.9 & 22.6 & 38.8 & 50.0 \\ % pvt
% ViL-T \cite{zhang2021ViL} & 27  % csin
%     & 41.4 & 63.5 & 45.0 & 24.5 & 44.5 & 55.4 
%     & 17
%     & 40.7 & 61.3 & 43.3 & 26.7 & 44.8 & 53.6 \\
CycleMLP-B1 \cite{chen2022cyclemlp} & 35  % flops: our
    & 39.4 & 61.4 & 43.0 & 36.8 & 58.6 & 39.1 
    & 25
    & 38.6 & 59.1 & 40.8 & 21.9 & 41.8 & 50.7  \\ % wavemlp 
WaveMLP-T \cite{tang2021imagewavemlp} & 35 
    & 41.5 & 63.7 & 45.4 & 38.2 & 60.9 & 40.7
    & 25
    & 40.4 & 61.0 & 43.4 & 24.9 & 43.7 & 51.7  \\ % wavemlp
\oursxt & 35
    & \textbf{42.8} & 64.9 & 46.9 & \textbf{39.5} & 62.1 & 42.5
    & 25
    & \textbf{41.2} & 62.3 & 43.7 & 24.4 & 45.3 & 54.2 \\ % done
\hline


ResNet-50 \cite{he2016deepresnet} & 44 % cswin 
    & 38.0 & 58.6 & 41.4 & 34.4 & 55.1 & 36.7
    & 38
    & 36.3 & 55.3 & 38.6 & 19.3 & 40.0 & 48.8 \\  % twins | flop:our
PVT-S \cite{wang2021pyramidpvt} & 44 % cswin 
    & 40.4 & 62.9 & 43.8 & 37.8 & 60.1 & 40.3 
    & 34
    & 40.4 & 61.3 & 43.0 & 25.0 & 42.9 & 55.7 \\ % ppvt
Swin-T \cite{liu2021swin} & 48 % cswin 
    & 42.2 & 64.6 & 46.2 & 39.1 & 61.6 & 42.0 
    & 29
    & 41.5 & 62,1 & 44.2 & 25.1 & 44.9 & 55.5 \\ % twins
TwinsP-S \cite{chu2021twins} & 44 % cswin 
    & 42.9 & 65.8 & 47.1 & 40.0 & 62.7 & 42.9 
    & 34
    & 43.0 & 64.1 & 46.0 & 27.5 & 46.3 & 57.3 \\ % twins
Twins-S \cite{chu2021twins} & 44 % cswin
    & 43.4 & 66.0 & 47.3 & 40.3 & 63.2 & 43.4 
    & 34
    & 43.0 & 64.2 & 46.3 & 28.0 & 46.4 & 57.5 \\ % twins
% PVTv2-B2 \cite{wang2021pvtv2} & 45 & - 
    % & 45.3 & 67.1 & 49.6 & 41.2 & 64.2 & 44.4 
    % & & & & & & \\ % pvtv2
% ViL-S \cite{zhang2021ViL} & 45 % csin
%     & 44.9 & 67.1 & 49.3 & 41.0 & 64.2 & 44.1 
%     & 36 % github
%     & 44.2 & 65.2 & 47.6 & 28.8 & 48.0 & 57.8 \\ 
% AS-MLP-T \cite{lian2021asmlp} & 48
%     &- &- &- &- &- &-
%     & -
%     &- &- &- &- &- &- \\ % asmlp
CycleMLP-B2 \cite{chen2022cyclemlp} & 47 % flops: our
    & 42.1 & 64.0 & 45.7 & 38.9 & 61.2 & 41.8 
    & 37
    & 40.9 & 61.8 & 43.4 & 23.4 & 44.7 & 53.4  \\ % cycle
WaveMLP-S \cite{tang2021imagewavemlp} & 47 
    & 44.0 & 65.8 & 48.2 & 40.0 & 63.1 & 42.9 
    & 37
    & 43.4 & 64.4 & 46.5 & 26.6 & 47.1 & 57.1 \\ % wavemlp
% Shift-T \cite{wang2022shift} & 48 & -
%     & 45.4 & -    & -    & 40.9 & -    & - 
%     & 47.1 & - & - & 42.3 & - & - \\ % shift
\ourst & 47
    & \textbf{44.8} & 66.9 & 49.0 & \textbf{41.0} & 64.2 & 44.3
    & 37
    & \textbf{43.6} & 64.9 & 46.8 & 27.2 & 47.5 & 57.9 \\ % done
\hline

ResNet-101 \cite{he2016deepresnet} & 63 % cswin
    & 40.4 & 61.1 & 44.2 & 36.4 & 57.7 & 38.8
    & 57 
    & 38.5 & 57.8 & 41.2 & 21.4 & 42.6 & 51.1 \\
PVT-M \cite{wang2021pyramidpvt} & 64  % cswin
    & 42.0 & 64.4 & 45.6 & 39.0 & 61.6 & 42.1
    & 54
    & 41.9 & 63.1 & 44.3 & 25.0 & 44.9 & 57.6 \\
TwinsP-B \cite{chu2021twins} & 64 % cswin
    & 44.6 & 66.7 & 48.9 & 40.9 & 63.8 & 44.2
    & 54
    & 44.3 & 65.6 & 47.3 & 27.9 & 47.9 & 59.6 \\
% ViL-M \cite{zhang2021ViL} & 60  % csin
%     & 43.4 & - & - & 39.7 & - & - 
%     & -
%     & - &- &- &- &- &- \\
Swin-S \cite{liu2021swin} & 69 % cswin
    & 44.8 & 66.6 & 48.9 & 40.9 & 63.4 & 44.2
    & 60
    & 44.5 & 65.7 & 47.5 & 27.4 & 48.0 & 59.9 \\
Twins-B \cite{chu2021twins} & 76  % cswin
    & 45.2 & 67.6 & 49.3 & 41.5 & 64.5 & 44.8
    & 67
    & 45.3 & 66.7 & 48.1 & 28.5 & 48.9 & 60.6 \\
CycleMLP-B3 \cite{chen2022cyclemlp} & 58 % wave | flops: our
    & 43.4 & 65.0 & 47.7 & 39.5 & 62.0 & 42.4
    & 48
    & 42.5 & 63.2 & 45.3 & 25.2 & 45.5 & 56.2 \\
WaveMLP-M \cite{tang2021imagewavemlp} & 60 
    & 45.3 & 67.0 & 49.5 & 41.0 & 64.1 & 44.1
    & 49
    & 44.8 & 65.8 & 47.8 & 28.0 & 48.2 & 59.1 \\
\ourss & 58
    & 46.0 & 68.2 & 50.4 & 42.0 & 65.3 & 45.5
    & 48
    & \textbf{45.4} & 66.7 & 48.5 & 28.3 & 49.7 & 59.7 \\
\arrayrulecolor{white}\hline
\oursb & 72
    & \textbf{46.5} & 68.6 & 51.0 & \textbf{42.5} & 66.1 & 45.8 
    & 62
    & 45.2 & 66.7 & 48.4 & 28.1 & 49.1 & 59.9 \\
\arrayrulecolor{black}\hline


X101-64 \cite{xie2017ResNeXt} & 102  % our
    & 42.8 & 63.8 & 47.3 & 38.4 & 60.6 & 41.3
    & 96
    & 41.0 & 60.9 & 44.0 & 23.9 & 45.2 & 54.0 \\ % cswin
PVT-L \cite{wang2021pyramidpvt} & 81 % cswin
    & 42.9 & 65.0 & 46.6 & 39.5 & 61.9 & 42.5 
    & 71
    & 42.6 & 63.7 & 45.4 & 25.8 & 46.0 & 58.4 \\
% ViL-B \cite{zhang2021ViL} & 76 % csin
%     & 45.1 & - & - & 41.0 & - & - 
%     & 
%     & 45.7 & 67.2 & 49.9 & 41.3 & 64.4 & 44.5 \\
TwinsP-L \cite{chu2021twins} & 81 
    & 45.4 & - & - & 41.5 & - & -
    & 71
    & 45.1 & 66.4 & 48.4 & - & - & - \\
Twins-L \cite{chu2021twins} & 120 
    & 45.9 & - & - & 41.6 & - & -
    & 111
    & 45.7 & 67.1 & 49.2 & - & - & - \\
Swin-B \cite{liu2021swin} & 107
    & 45.5 & - & - & 42.1 & - & -
    & 98
    & 44.7 & 65.9 & 47.8 & - & - & - \\
% CycleMLP-B4 \cite{chen2022cyclemlp} & 72 % wave | flops: our
%     & 44.1 & 65.7 & 48.1 & 40.2 & 62.7 & 43.5
%     & 62
%     & 43.2 & 63.9 & 46.2 & 26.6 & 46.5 & 57.4 \\
CycleMLP-B5 \cite{chen2022cyclemlp} & 95  % wave | flops: our flops: our
    & 44.1 & 65.5 & 48.4 & 40.1 & 62.8 & 43.0
    & 86
    & 42.7 & 63.3 & 45.3 & 24.1 & 46.3 & 57.4  \\
WaveMLP-B \cite{tang2021imagewavemlp} & 75
    & 45.7  & 67.5 & 50.1 & 27.8 & 49.2 & 59.7
    & 66
    & 44.2 & 65.1 & 47.1 & 27.1 & 47.8 & 58.9 \\


\oursl & 96
    & \textbf{47.4} & 69.9 & 52.0 & \textbf{43.2} & 67.3 & 46.5
    & 86
    & \textbf{46.1} & 67.4 & 49.4 & 29.9 & 50.1 & 61.0 \\

\hline
% \Block{1-15}{}&&&&&&&&&&&&&&\\[-0.5cm]
% \Block{1-15}{}&&&&&&&&&&&&&&\\
% \hline
% \Block{1-1}{} & \Block{1-7}{Mask R-CNN 1$\times$ MS} & & &&&&& \Block{1-7}{RetinaNet 3$\times$} &&&&&&\\
% \hline

% \oursxt & 35
%     &42.9 & 65.5 & 47.0 & 39.3 & 62.3 & 42.1
%     & 25
%     & 43.7 & 64.7 & 46.7 & 28.9 & 47.4 & 57.4  \\
% \hline

% Swin-T \cite{liu2021swin} & 48
%     & 43.7 & 66.6 & 47.7 & 39.8 & 63.3 & 42.7 % github
%     & 39
%     & 45.0 & 65.9 & 48.4 & 29.7 & 48.9 & 58.1 \\ % focal
% % TwinP-S \cite{chu2021twins} & -
% %     & - & - & - & - & - & -
% %     & 34
% %     & 45.2 & 66.5 & 48.6 & 30.0 & 48.8 & 58.9 \\
% % Twin-S \cite{chu2021twins} & -
% %     & - & - & - & - & - & - 
% %     & 34
% %     & 45.6 & 67.1 & 48.6 & 29.8 & 49.3 & 60.0 \\
% \ourst & 47
%     & 45.8 & 68.3 & 50.3 & 41.6 & 65.2 & 44.2
%     & 37
%     & 45.8 & 66.9 & 49.2 & 29.9 & 49.3 & 59.9 \\
% \hline

% Swin-S \cite{liu2021swin} & 69
%     & 46.4 & - & - & 41.7 & - & - 
%     & 60 
%     & 46.4 & 67.0 & 50.1 & 31.0 & 50.1 & 60.3 \\ %focal
% % TwinsP-B \cite{chu2021twins} & -
% %     & - & - & - & - & - & - 
% %     & 54
% %     & 46.4 & 67.7 & 49.8 & 31.3 & 50.2 & 61.4 \\
% % Twins-B \cite{chu2021twins} & -
% %     & - & - & - & - & - & - 
% %     & 67
% %     & 46.9 & 68.0 & 50.2 & 31.7 & 50.3 & 61.8 \\
% \ourss & 58
%     & 46.8 & 69.2 & 51.4 & 42.5 & 66.3 & 45.8
%     & 47
%     & 45.7 & 67.3 & 48.8 & 30.0 & 50.0 & 59.5 \\
% \oursb & 72
%     & 47.0 & 69.6 & 51.7 & 42.7 & 66.6 & 46.0
%     & 62 
%     & 46.6 & 67.7 & 50.1 & 30.4 & 50.4 & 61.0 \\
% \hline

% Swin-B \cite{liu2021swin} & 107
%     & 46.9 &- & -&42.1 & - & -
%     & 98 
%     & 45.8 & 66.4 & 49.1 & 29.9 & 49.4 & 60.3 \\ %focal
% \oursl & 96
%     & 47.4 & 70.2 & 52.2 & 43.0 & 67.1 & 46.0
%     & 86 
%     & 47.5 & 68.8 & 51.2 & 31.5 & 51.4 & 62.0 \\
% \hline

\end{NiceTabular}
}
% \subcaption{Mask R-CNN 1$\times$ and RetinaNet 1$\times$.}
% \end{subtable}

% \vspace{-1cm}






% \quad

% \begin{subtable}[t]{\linewidth}



% \begingroup

% % \begi
% \resizebox{\textwidth}{!}{    
% \begin{NiceTabular}{@{}l@{}|@{}c@{}|ccc|ccc|@{}c@{}|ccc|ccc@{}}
% \CodeBefore
% \rectanglecolor{\rc}{4-1}{4-}
% \rectanglecolor{\rc}{7-1}{7-}
% \rectanglecolor{\rc}{10-1}{11-}
% \rectanglecolor{\rc}{14-1}{14-}
% \Body
% \hline
% \multirow{2}{*}{Model} &  \multicolumn{7}{c}{Mask R-CNN 1$\times$ MS} & \multicolumn{7}{c}{RetinaNet 3$\times$} \\
% \cline{2-8}
% \cline{9-15}
%   & 
%   \begingroup
%   \scriptsize
%   \#P/M
%   \endgroup
%   & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$^m$ & AP$^m_{50}$ & AP$^m_{75}$ & 
%   \begingroup
%   \scriptsize
%   \#P/M
%   \endgroup
%   & AP$^b$ & AP$^b_{50}$ & AP$^b_{75}$ & AP$_S$ & AP$_{M}$ & AP$_{L}$ \\
% \hline

% PVT-T \cite{wang2021pyramidpvt} & -
%     & - & - & - & - & - & -
%     & 23
%     & 39.4 & 59.8 & 42.0 & 25.5 & 42.0 & 52.1 \\
% \oursxt & 35
%     & 42.9 & 65.5 & 47.0 & 39.3 & 62.3 & 42.1
%     & 25
%     & \textbf{43.7} & 64.7 & 46.7 & 28.9 & 47.4 & 57.4  \\
% \hline

% PVT-S \cite{wang2021pyramidpvt} & -
%     & - & - & - & - & - & -
%     & 34
%     & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2 \\
% Swin-T \cite{liu2021swin} & 48
%     & 43.7 & 66.6 & 47.7 & 39.8 & 63.3 & 42.7 % github
%     & 39
%     & 45.0 & 65.9 & 48.4 & 29.7 & 48.9 & 58.1 \\ % focal
% % TwinP-S \cite{chu2021twins} & -
% %     & - & - & - & - & - & -
% %     & 34
% %     & 45.2 & 66.5 & 48.6 & 30.0 & 48.8 & 58.9 \\
% % Twin-S \cite{chu2021twins} & -
% %     & - & - & - & - & - & - 
% %     & 34
% %     & 45.6 & 67.1 & 48.6 & 29.8 & 49.3 & 60.0 \\
% \ourst & 47
%     & \textbf{45.8} & 68.3 & 50.3 & \textbf{41.6} & 65.2 & 44.2
%     & 37
%     & \textbf{45.8} & 66.9 & 49.2 & 29.9 & 49.3 & 59.9 \\
% \hline

% PVT-M \cite{wang2021pyramidpvt} & -
%     & - & - & - & - & - & -
%     & 54
%     & 43.2 & 63.8 & 46.1 & 27.3 & 46.3 & 58.9 \\
% Swin-S \cite{liu2021swin} & 69
%     & 46.4 & - & - & 41.7 & - & - 
%     & 60 
%     & 46.4 & 67.0 & 50.1 & 31.0 & 50.1 & 60.3 \\ %focal
% % TwinsP-B \cite{chu2021twins} & -
% %     & - & - & - & - & - & - 
% %     & 54
% %     & 46.4 & 67.7 & 49.8 & 31.3 & 50.2 & 61.4 \\
% % Twins-B \cite{chu2021twins} & -
% %     & - & - & - & - & - & - 
% %     & 67
% %     & 46.9 & 68.0 & 50.2 & 31.7 & 50.3 & 61.8 \\
% \ourss & 58
%     & 46.8 & 69.2 & 51.4 & 42.5 & 66.3 & 45.8
%     & 47
%     & 46.3 & 68.0 & 49.5 & 30.4 & 50.6 & 59.9 \\
% \arrayrulecolor{white}\hline
% \oursb & 72
%     & \textbf{47.0} & 69.6 & 51.7 & \textbf{42.7} & 66.6 & 46.0
%     & 62 
%     & \textbf{46.6} & 67.7 & 50.1 & 30.4 & 50.4 & 61.0 \\
% \arrayrulecolor{black}\hline

% PVT-L \cite{wang2021pyramidpvt} & -
%     & - & - & - & - & - & -
%     & 71
%     & 43.4 & 63.6 & 46.1 & 26.1 & 46.0 & 59.5 \\
% Swin-B \cite{liu2021swin} & 107
%     & 46.9 &- & -&42.1 & - & -
%     & 98 
%     & 45.8 & 66.4 & 49.1 & 29.9 & 49.4 & 60.3 \\ %focal
% \oursl & 96
%     & \textbf{47.4} & 70.3 & 52.4 & \textbf{43.1} & 67.5 & 46.2
%     & 86 
%     & \textbf{47.5} & 68.8 & 51.2 & 31.5 & 51.4 & 62.0 \\
% \hline

% \end{NiceTabular}
% }
% \subcaption{Mask R-CNN 1$\times$ MS and RetinaNet 3$\times$.}
% \endgroup


% \end{subtable}




\vspace{-0.3cm}
\endgroup

==> tables/supp_ablation_atm.tex <==

\begingroup

\setlength{\tabcolsep}{3pt}
\begin{NiceTabular}{@{}lcclcl@{}}[code-before=
\rectanglecolor{\rc}{4-2}{4-6}
\rectanglecolor{\rc}{6-2}{6-6}
\rectanglecolor{\rc}{8-2}{8-6}
]

\hline
& & \multicolumn{2}{c}{Semantic FPN} & \multicolumn{2}{c}{Mask R-CNN} \\
Backbone & Neck & FLOPS & mIoU & FLOPS & AP$^b$ \\
\hline

\multirow{2}{*}{\ourst}
& FPN         & 42.4 & 45.8
            & 251.1 & 44.8 \\
& ATMFPN  
    & 41.4 & 46.5\tcg{\large$_{\uparrow0.7}$}
    & 247.0 & 45.6\tcg{\large$_{\uparrow0.8}$}   \\
\hline
\end{NiceTabular}
\endgroup
